The Entropy of Floating-Point Numbers

Here we present an analytic approximation for the entropy of floating-point numbers, along with bounds on the error of this approximation. It is well-known that the differential entropy is tightly linked to the discrete entropy of a uniformly quantized random variable. Our approximation uncovers a different quantity that provides this link for floating-point quantization. Additionally, we prove that the entropy of a floating-point quantized random variable is approximately unchanged under scaling. Closed-form expressions for the floating-point entropy of common distributions are provided and compared to exact results.

==> appendices/approx_entropy.tex <==
\section{Approximating the entropy of floating point numbers}\label{app:FPN}

Here we review the details of calculations used to approximate the entropy of floating point numbers. 









\subsubsection*{Approximation 1 -- Relating discrete and differential entropy for non-uniform bins}\label{app:FPN_app1}

Let there be a quantization scheme with $K$ representable values
$\{u_1, u_2, \ldots, u_K\}$, where $u_1 < u_2 < \cdots < u_K$.
Let $\Xv \sim f_\Xv$, where $f_\Xv$ is a differentiable probability density function with support on
\begin{equation}
\mathbb{U}^d \triangleq \left[-2^{e_{max} + 1} + 2^{e_{max} - p}, \,\, 2^{e_{max} + 1} - 2^{e_{max} - p}\right]^d,
\end{equation}
where we assume each component $X_j$ is independently clipped and quantized.

Let $\Delta: \left[-2^{e_{max} + 1} + 2^{e_{max} - p},\,\, 2^{e_{max} + 1} - 2^{e_{max} - p}\right] \to \mathbb{R}_+$
encode the bin sizes of the quantization scheme for a single component, where
\begin{equation*}
    \begin{aligned}
    \Delta(x_j) &\triangleq \sum_{i=2}^{K-1}\frac{u_{i+1} - u_{i-1}}{2}
    \indic{x_j \in \Big[\frac{u_i+u_{i-1}}{2}, \frac{u_{i+1}+u_i}{2}\Big)} + (u_2 - u_1)\indic{x_j \in [-2^{e_{max} + 1} + 2^{e_{max} - p}, \frac{u_{2} + u_{1}}{2}]}\nonumber\\
    & + (u_K - u_{K-1})\indic{x_j \in [\frac{u_{K} + u_{K-1}}{2}, 2^{e_{max} + 1} - 2^{e_{max} - p}]}.
    \end{aligned}
\end{equation*}
Since each component is stored on its own floating-point register, the quantization cell for $\Xv_Q$ is a $d$-dimensional rectangle with volume
\begin{equation}
\bDelta(\xv) \triangleq \prod_{j=1}^{d} \Delta(x_j),
\qquad
\log \bDelta(\xv) = \sum_{j=1}^{d} \log \Delta(x_j).
\end{equation}

Let $\mathbf{i} = (i_1,\dots,i_d)$ index the $d$-dimensional quantization cells, where $i_j \in \{1,\dots,K\}$. Define the cell boundaries
\begin{equation}
a_i=\begin{cases}
-2^{e_{max} + 1} + 2^{e_{max} - p} & i=1\\[2pt]
\frac{u_i+u_{i-1}}2 & 2\leq i\leq K
\end{cases},
\qquad
b_i=\begin{cases}
\frac{u_{i+1}+u_i}2 & 1\leq i\leq K-1\\[2pt]
2^{e_{max} + 1} - 2^{e_{max} - p} & i=K.
\end{cases}
\end{equation}
For each $d$-dimensional index $\mathbf{i}$, define the quantization cell
\begin{equation}
B_{\mathbf{i}} \triangleq \prod_{j=1}^d [a_{i_j}, b_{i_j}],
\end{equation}
and let
\begin{equation}
p_{\mathbf{i}} \triangleq \mathbb{P}\{\Xv\in B_{\mathbf{i}}\}
= \mathbb{P}\{\Xv_Q = \mathbf{u}_{\mathbf{i}}\},
\end{equation}
where $\mathbf{u}_{\mathbf{i}}$ is the $d$-dimensional representable value corresponding to the quantization cell $B_\mathbf{i}$.

Then the discrete entropy of $\Xv_Q$ is
\begin{equation}
H(\Xv_Q) = -\sum_{\mathbf{i}} p_{\mathbf{i}} \log p_{\mathbf{i}}.
\end{equation}

To relate this discrete entropy to the differential entropy of $\Xv$, define the piecewise-uniform density
\begin{equation}
g(\xv)
\triangleq
\sum_{\mathbf{i}}
\frac{p_{\mathbf{i}}}{|B_{\mathbf{i}}|}
\indic{\xv\in B_{\mathbf{i}}},
\label{eq:piecewise_uniform_g}
\end{equation}
where $|B_{\mathbf{i}}| = \bDelta(\xv)$ for $\xv \in B_{\mathbf{i}}$ is the volume of each rectangular cell $B_{\mathbf{i}}$. By construction, $g$ is constant on each cell and integrates to one across all cells.

Following \cite{kostina_data_2017}, we can derive an exact identity relating the discrete and differential entropies. By the definition of Kullback-Leibler divergence,
\begin{align}
\relent{f_{\Xv}}{g}
&=
\int_{\mathbb{U}^d}
f_{\Xv}(\xv)
\log\frac{f_{\Xv}(\xv)}{g(\xv)}
\,d\xv
\notag\\
&=
\int_{\mathbb{U}^d}
f_{\Xv}(\xv)\log f_{\Xv}(\xv)
\,d\xv
-
\int_{\mathbb{U}^d}
f_{\Xv}(\xv)\log g(\xv)
\,d\xv
\notag\\
&=
-h(\Xv)
-
\int_{\mathbb{U}^d}
f_{\Xv}(\xv)\log g(\xv)
\,d\xv.
\label{eq:KL_start}
\end{align}
Since $g(\xv) = p_{\mathbf{i}}/|B_{\mathbf{i}}|$ for $\xv\in B_{\mathbf{i}}$,
\begin{align}
\int_{\mathbb{U}^d}
f_{\Xv}(\xv)\log g(\xv)
\,d\xv
&=
\sum_{\mathbf{i}}
\int_{B_{\mathbf{i}}}
f_{\Xv}(\xv)
\log\left(\frac{p_{\mathbf{i}}}{|B_{\mathbf{i}}|}\right)
d\xv\\
&=
\sum_{\mathbf{i}}
 \bigg(
\int_{B_{\mathbf{i}}}
f_{\Xv}(\xv) d\xv\bigg)
\log\left(\frac{p_{\mathbf{i}}}{|B_{\mathbf{i}}|}\right)
=
\sum_{\mathbf{i}}
p_{\mathbf{i}}
\log\left(\frac{p_{\mathbf{i}}}{|B_{\mathbf{i}}|}\right)\\
&=
\sum_{\mathbf{i}} p_{\mathbf{i}}\log p_{\mathbf{i}}
-
\sum_{\mathbf{i}} p_{\mathbf{i}}\log |B_{\mathbf{i}}|.
\label{eq:KL_middle}
\end{align}
Substituting Eq.~\eqref{eq:KL_middle} into Eq.~\eqref{eq:KL_start} yields
\begin{align}
\relent{f_{\Xv}}{g}
&=
-h(\Xv)
-
\sum_{\mathbf{i}} p_{\mathbf{i}}\log p_{\mathbf{i}}
+
\sum_{\mathbf{i}} p_{\mathbf{i}}\log |B_{\mathbf{i}}|
\notag\\
&=
-h(\Xv)
+
H(\Xv_Q)
+
\mathbb{E}[\log \bDelta(\Xv)],
\end{align}
or equivalently,
\begin{equation}
H(\Xv_Q)
=
h(\Xv)
-
\mathbb{E}[\log \bDelta(\Xv)]
+
\relent{f_{\Xv}}{g}.
\label{eq:exact_identity}
\end{equation}
Approximation 1 corresponds to neglecting the nonnegative correction term $\relent{f_{\Xv}}{g}$:
\begin{equation}
H(\Xv_Q)
\approx
h(\Xv)
-
\mathbb{E}[\log \bDelta(\Xv)].
\label{eq:approx1_clean}
\end{equation}

\cite{kostina_data_2017} shows rigorously that the correction term $\relent{f_{\Xv}}{g}$ becomes large if $f_{\Xv}$ varies noticeably within each quantization cell, and vanishes if the function is uniform across each cell. Here, we can understand this at a basic level by noting that $g(\xv)$ is equal to the mean value of $f_{\Xv}$ within a given bin $B_{\mathbf{i}}$. By the multivariate mean value theorem, $g(\xv) = f_\Xv(\mathbf{\tilde x_{\mathbf{i}}})$ for some $\mathbf{\tilde x}_{\mathbf{i}} \in B_{\mathbf{i}}$. Taylor expanding $f_{\Xv}(\xv)$ within cell $B_{\mathbf{i}}$ to first order around $\mathbf{\tilde x}_{\mathbf{i}}$ we see:
\begin{equation}
f_{\Xv}(\xv) \approx g (\xv)+ \nabla f_{\Xv}(\mathbf{\tilde x}_{\mathbf{i}}) \cdot (\xv- \mathbf{\tilde x}_{\mathbf{i}}).
\end{equation}
Since $\relent{f_{\Xv}}{g} \approx 0$ when $f_{\Xv} \approx g$, a cell can contribute significantly to the error if the size of the cell and the gradient of $f_{\Xv}$ are simultaneously large, since $(\xv-\mathbf{\tilde x}_{\mathbf{i}})$ is bounded by the size of the cell. However, when the cell diameter is small in regions where the density varies rapidly, or if the cell diameter is large where the density varies only slowly, the discrepancy between $f_{\Xv}$ and its cell average $g(\xv)$ remains small.

Finally, we can note that if each component is quantized independently, then
\begin{equation}
\mathbb{E}[\log \bDelta(\Xv)]
=
\sum_{j=1}^{d}\mathbb{E}_{X_j}[\log \Delta(X_j)],
\label{eq:separable}
\end{equation}
so that Approximation 1 takes the form
\begin{equation}
\tilde{H}(\Xv_Q)
\triangleq
h(\Xv)
-
\sum_{j=1}^{d}\mathbb{E}_{X_j}[\log \Delta(X_j)].
\label{eq:multi_var_diff_disc}
\end{equation}










\subsubsection*{Approximation 2 -- Smoothing the bin size function and extending its domain}\label{app:FPN_app2}

In the multivariate case, with $\Delta_s(x) = \frac{|x|}{\sqrt{2}}\cdot 2^{1-p}$ from Eq.~\eqref{eq:step_approx}, we can define
\begin{equation}
    \bDeltas(\xv) = \prod^d_{j=1} \Delta_s(x_j).
\end{equation}
Again, $\mathbb{U}^d = [-2^{e_{max} + 1} + 2^{e_{max} - p}, \,\, 2^{e_{max} + 1} - 2^{e_{max} - p}]^d$, where $e_{max} = 2^{E-1}$. Assuming that the tails of $f_\Xv$ are vanishingly small,
\begin{equation}
    \int_{\mathbb{R}^d \setminus \mathbb{U}^d} f_\Xv(\xv) \, d\xv \approx 0,
\end{equation}
we extend the domain from $\mathbb{U}^d$ to $\mathbb{R}^d$. As noted in the main text, this extension requires that the omitted tail integral $\int_{\mathbb{R}^d\setminus\mathbb{U}^d} f_\Xv(\xv)|\log[f_\Xv(\xv)\bDeltas(\xv)]|\,d\xv$ is near zero, not merely that the tail mass is small. For the Gaussian and Student's $t$ distributions used in this paper, the tail decay dominates the linear growth of $\Delta_s$, so this tail integral is negligible when the granular region $\mathbb{U}$ is sufficiently large (i.e., $E$ is not too small). With this we can say from Eq.~\eqref{eq:multi_var_diff_disc} $\tilde H(\Xv_Q) \approx \tilde H_s(\Xv_Q)$, where
\begin{equation}
    \tilde H_s(\Xv_Q) = -\int_{\mathbb{R}^d}  f_\Xv(\xv)
    \log\left[f_\Xv(\xv)
    \prod_{j=1}^d \Delta_s(x_j)\right] d\xv.
\end{equation}













Define the smooth-bin approximation restricted to $\mathbb U^d$ as
\begin{equation}
\label{eq:Ht_s_U}
\tilde H_{s,\mathbb U}(\Xv_{fp})
\;\triangleq\;
-\int_{\mathbb U^d} f_{\Xv}(\xv)\,\log\left[f_{\Xv}(\xv)\prod_{j=1}^d \Delta_s(x_j)\right]d\xv.
\end{equation}
Theorem~\ref{thm:steps} bounds the smoothing error by the $d/2$ term plus the explicit contribution from the bins adjacent to zero.

Define the special-bin set
\begin{equation}
\label{eq:special_bins}
\begin{aligned}
\mathcal B_0 &\triangleq \left\{x\in \mathbb U:\ |x|<2^{e_{\min}}(1+2^{-p})\right\}
\end{aligned}
\end{equation}
where $\mathcal B_0$ is the union of the two bins adjacent to $0$. When $x \in \mathcal B_{0}$, $\Delta(x) = \Delta_0 = 2^{e_{\min}}(1+2^{-p})$. Define
\begin{equation}
\label{eq:special_error}
\varepsilon_{0}(\Xv)
\triangleq
\sum_{j=1}^{d}
\int_{\mathcal B_{0}}
f_{X_j}(x)
\left|
\log\bracket{\frac{\Delta_s(x)}{\Delta_0}}
\right|dx.
\end{equation}

\begin{theorem}[Error bound for smoothing the bin-size function]\label{thm:steps}
Let $\Xv\sim f$ be a $d$-dimensional random vector with the probability density $f$ supported on $\mathbb U^d$, and let $X_j$ denote its $j$th component. Let $\tilde H(\Xv_{fp})$ be the approximation from App.~\ref{app:FPN_app1} using the true midpoint bin-size function $\Delta$, and let $\tilde H_{s,\mathbb U}(\Xv_{fp})$ be the corresponding approximation on $\mathbb U^d$ using $\Delta_s$. Then
\begin{equation}
\abs{\tilde H(\Xv_{fp}) - \tilde H_{s,\mathbb U}(\Xv_{fp})} \leq \frac{d}{2} + \varepsilon_{0}(\Xv),
\end{equation}
where $\varepsilon_{0}(\Xv)$ is finite and defined in Eq.~\eqref{eq:special_error}.
\end{theorem}

\begin{proof}

There are 3 types of bins for which we will bound the error: bins on the interior of an exponent block, bins on the outer edges, and bins on the boundary between exponent blocks (regions for which a single exponent value applies). The bound can be shown by considering the ratio between bin sizes, case by case.

\paragraph{Interior Bins}
For interior bins strictly within each exponent block $e$, by Eq.~\eqref{eq:true_bins},
\begin{equation}
    \label{eq:real_bins}
    \Delta(x_j) = 2^{e-(p-1)} \quad \text{for } 2^e \leq |x_j| < 2^{e+1},
\end{equation}
and within this range $\Delta_s(x_j) = \frac{|x_j|}{\sqrt{2}} \cdot 2^{1-p}$ satisfies
\begin{equation}
    \begin{aligned}
    &\frac{2^e}{\sqrt{2}}2^{1-p} \leq \Delta_s(x_j) \leq \frac{2^{e+1}}{\sqrt{2}}2^{1-p}\\
    \implies &\frac{1}{\sqrt{2}} \leq \frac{\Delta_s(x_j)}{\Delta(x_j)} < \sqrt{2}.
    \end{aligned}
\end{equation}

\paragraph{Outer clipping bins}

For the outer clipping bins, by symmetry it suffices to analyze $[\frac{u_K + u_{K-1}}{2}, 2^{e_{\max}+1}-2^{e_{\max}-p}]$ which is the bin on positive side of the real line. When $p \geq 2$, we know that $u_K = 2^{e_{max}+1}(1 - 2^{-p})$, and $u_{K-1} = 2^{e_{max}+1}(1 - 2^{1-p})$, so the outer clipping bin size is \begin{equation}
\Delta(x_j) = 2^{e_{max} + 1} - 2^{e_{max} - p}- \frac{u_K + u_{K-1}}{2} = 2^{e_{max}}\paren{2^{1-p}} = 2^{e_{max}-p + 1}
\end{equation}
Now, we have
\begin{equation}
\begin{aligned}
  &\frac{(u_K + u_{K-1})}{2\sqrt{2}}2^{1-p} \leq \Delta_s(x_j) \leq \frac{2^{e_{max} + 1} - 2^{e_{max} - p}}{\sqrt{2}}2^{1-p}\\
  \implies &\frac{ 2^{e_{max}}(1 - 2^{-1-p} - 2^{-p})}{2^{e_{max} - p}\sqrt{2}}2^{1-p} \leq \frac{\Delta_s(x_j)}{\Delta(x_j)} \leq \frac{2^{e_{max}}(1 - 2^{-1 - p})}{2^{e_{max} - p}\sqrt{2}}2^{1-p}\\
  \implies &\frac{ 2(1 - 2^{-1-p} - 2^{-p})}{\sqrt{2}} \leq \frac{\Delta_s(x_j)}{\Delta(x_j)} \leq \frac{2(1- 2^{-1-p})}{\sqrt{2}}\\
  \implies &\sqrt{2}(1 - 2^{-1-p} - 2^{-p}) \leq \frac{\Delta_s(x_j)}{\Delta(x_j)} \leq \sqrt{2}(1- 2^{-1-p}).
\end{aligned}
\end{equation}
When $p = 1$, $u_K = 2^{e_{max}}$ and $u_{K-1} = 2^{e_{max}-1}$. The true bin width is 
\begin{equation}
\Delta(x_j) = 2^{e_{max}+1} - 2^{e_{max}-1} - \frac{1}{2}(2^{e_{max}} + 2^{e_{max}-1}) = 3\cdot2^{e_{max}-2}.
\end{equation}
Using the same bounding technique, we have
\begin{equation}
\begin{aligned}
  &\frac{2^{e_{max}} + 2^{e_{max}-1}}{2\sqrt{2}} \leq \Delta_s(x_j) \leq \frac{2^{e_{max}+1} - 2^{e_{max}-1}}{\sqrt{2}}\\
  \implies &\frac{3\cdot 2^{e_{max}-2}}{3\cdot2^{e_{max}-2}\sqrt{2}} \leq \frac{\Delta_s(x_j)}{\Delta(x_j)} \leq \frac{3\cdot 2^{e_{max}-1}}{3\cdot2^{e_{max}-2}\sqrt{2}}\\
  \implies &\frac{ 1}{\sqrt{2}} \leq \frac{\Delta_s(x_j)}{\Delta(x_j)} \leq \frac{2}{\sqrt{2}}.
\end{aligned}
\end{equation}
For the outer clipping bins, we see that for all $p\geq 1$, $\frac{1}{\sqrt{2}} \leq \frac{\Delta_s(x_j)}{\Delta(x_j)} \leq \sqrt{2}$.

\paragraph{Exponent boundary bins}

At exponent boundaries, let the last representable value of the $e$-th exponent block be $u_A = 2^{e+1} - 2^{e-(p-1)}$. the first representable value of the $e+1$-th exponent block be $u_B = 2^{e+1}$, and the second representable value of the $e+1$-th exponent block be $u_C = 2^{e+1} + 2^{e+1 - (p-1)}$. The left boundary of the midpoint-quantization bin for $u_B$ is $m_L = \frac{u_A + u_B}{2} = 2^{e+1}(1 - 2^{-p-1})$ while the right boundary is $m_R = \frac{u_B + u_C}{2} = 2^{e+1}(1+2^{-p})$. When $x_j \in [m_L, m_R)$, the bin width is
\begin{equation}\label{eq:exp_boundary}
\Delta(x_j) = m_R - m_L = 3 \cdot 2^{e-p},
\end{equation}
and the ratio $\Delta_s(x_j)/\Delta(x_j)$ is bounded by
\begin{equation}
    \begin{aligned}
    &\frac{2^{e+1}(1 - 2^{-p-1})}{\sqrt{2}}2^{1-p} \leq \Delta_s(x_j) \leq \frac{2^{e+1}(1+2^{-p})}{\sqrt{2}}2^{1-p}\\
    \implies & \frac{2^{e+1}(1 - 2^{-p-1})}{3 \cdot 2^{e-p}\sqrt{2}}2^{1-p} \leq \frac{\Delta_s(x_j)}{\Delta(x_j)} \leq \frac{2^{e+1}(1+2^{-p})}{3 \cdot 2^{e-p}\sqrt{2}}2^{1-p}\\
    \implies & \frac{2\sqrt{2}(1 - 2^{-p-1})}{3} \leq \frac{\Delta_s(x_j)}{\Delta(x_j)}  \leq \frac{2\sqrt{2}(1+2^{-p})}{3}.
    \end{aligned}
\end{equation}
When $p = 1$ the lower bound is equal to $1/\sqrt{2}$ and the upper bound is equal to $\sqrt{2}$. The lower bound is monotonically increasing in $p$ while the upper bound is monotonically decreasing in $p$, and both converge to $2\sqrt{2}/3$ as $p \rightarrow \infty$, which is between $1/\sqrt{2}$ and $\sqrt{2}$. This means both bounds lie within $[1/\sqrt{2},\, \sqrt{2}]$, so for within exponent block bins and exponent boundary bins,
\begin{equation}
    -\frac{1}{2} \leq \log\left[\frac{\Delta_s(x_j)}{\Delta(x_j)}\right] < \frac{1}{2}.
\end{equation}

\paragraph{Bound on entropy difference from bin ratios}


Hence, for every $x_j\in \mathbb U\setminus \mathcal B_{0}$,
\begin{equation}
\abs{\log\bracket{\frac{\Delta_s(x_j)}{\Delta(x_j)}}} \leq \frac{1}{2}.
\end{equation}

The remaining points are exactly the special bins collected in $\mathcal B_{0}$, where we do not claim a uniform pointwise bound and instead keep their contribution explicitly:
\begin{equation}
\begin{aligned}
&\left|
\tilde H(\Xv_{fp}) - \tilde H_{s,\mathbb U}(\Xv_{fp}) \right| = \Bigg | -\int_{\mathbb U^d} f_{\Xv}(\xv)\,\log\left[f_{\Xv}(\xv)\prod_{j=1}^d \Delta(x_j)\right]d\xv  \\ & \qquad \qquad \qquad \qquad \qquad
+ \int_{\mathbb U^d} f_{\Xv}(\xv)\,\log\left[f_{\Xv}(\xv)\prod_{j=1}^d \Delta_s(x_j)\right]d\xv \Bigg |\\
&\left|
\tilde H(\Xv_{fp}) - \tilde H_{s,\mathbb U}(\Xv_{fp}) \right| = \abs{\sum_{j=1}^{d} \Esub{\log\bracket{\frac{\Delta_s(x)}{\Delta(x)}}}{X_j}} \\
&\leq\sum_{j=1}^{d} \int_{\mathbb U\setminus \mathcal B_{0}} f_{X_j}(x) \abs{\log\bracket{\frac{\Delta_s(x)}{\Delta(x)}}}dx + \varepsilon_{0}(\Xv) \leq\frac d2 + \varepsilon_{0}(\Xv).
\end{aligned}
\end{equation}
The point $x=0$ has measure zero, and $\varepsilon_{0}(\Xv)$ is finite since each marginal density is continuous on $\mathbb U$ while $|\log|x||$ is locally integrable near $0$.
\end{proof}

Not only is $\varepsilon_{0}(\Xv)$ finite, as shown in Theorem~\ref{thm:steps}, but for the probability distributions that this paper studies, Corollary~\ref{cor:eps_sp_bound} shows that $\varepsilon_{0}(\Xv)$ is negligibly small.


\begin{corollary}[Bound on $\varepsilon_{0}$ for densities bounded near zero]
\label{cor:eps_sp_bound}
Under the hypotheses of Theorem~\ref{thm:steps}, with
$\mathcal{B}_{0} = \mathcal{B}_0$ (the two zero-crossing bins),
define
\begin{equation}
  a \;\triangleq\; 2^{e_{\min}}\bigl(1 + 2^{-p}\bigr),
  \qquad
  C_0 \;\triangleq\; 2\,a\left(p - \frac{1}{2} + \log e\right).
\end{equation}
Then
\begin{equation}
\label{eq:eps_sp_general}
  \varepsilon_{0}(\Xv)
  \;\le\;
  C_0
  \sum_{j=1}^{d}
  \sup_{x \in \mathcal{B}_0} f_{X_j}(x).
\end{equation}
 
If every marginal density $f_{X_j}$ attains its mode at $0$,
then
\begin{equation}
\label{eq:eps_sp_mode}
  \varepsilon_{0}(\Xv)
  \;\le\;
  C_0
  \sum_{j=1}^{d} f_{X_j}(0).
\end{equation}
 
\medskip
\noindent\textbf{(i)\; Zero-mean Gaussian marginals.}\;
If $X_j \sim \mathcal{N}(0,\sigma_j^2)$, then $f_{X_j}(0) = 1/(\sigma_j\sqrt{2\pi})$, and
\begin{equation}
\label{eq:eps_sp_gauss}
  \varepsilon_{0}(\Xv)
  \;\le\;
  \frac{C_0}{\sqrt{2\pi}}
  \sum_{j=1}^{d} \frac{1}{\sigma_j}.
\end{equation}
 
\noindent\textbf{(ii)\; Scaled Student's $t$ marginals.}\;
If $X_j \sim t_\nu(0,\sigma_j)$ with density
$f_{X_j}(x)
= \frac{\Gamma\bigl(\frac{\nu+1}{2}\bigr)}
       {\sigma_j\sqrt{\nu\pi}\;\Gamma\bigl(\frac{\nu}{2}\bigr)}
  \bigl(1 + x^2/(\nu\sigma_j^2)\bigr)^{-(\nu+1)/2}$,
then $f_{X_j}(0) = \Gamma\bigl(\frac{\nu+1}{2}\bigr)
  \big/\bigl(\sigma_j\sqrt{\nu\pi}\;\Gamma\bigl(\frac{\nu}{2}\bigr)\bigr)$, and
\begin{equation}
\label{eq:eps_sp_student}
  \varepsilon_{0}(\Xv)
  \;\leq\;
  \frac{C_0\;\Gamma\bigl(\frac{\nu+1}{2}\bigr)}
       {\sqrt{\nu\pi}\;\Gamma\bigl(\frac{\nu}{2}\bigr)}
  \sum_{j=1}^{d} \frac{1}{\sigma_j}.
\end{equation}
\end{corollary}
 
\begin{proof}
We see that $a$ is the value of the first interior midpoint for positive bin adjacent to zero $(0, a]$. The true midpoint bin width is,
$\Delta(x_j) = a$,
while $\Delta_s(x_j) = x \cdot 2^{1-p}/\sqrt{2}$.
Since on this interval $x_j 2^{1-p}/\sqrt{2} \leq x_j \leq a$, the ratio $\Delta_s(x_j)/\Delta(x_j) < 1$
on the entire bin, so
\begin{equation}
  \abs{\log\bracket{\Delta_s(x)/\Delta(x)}}
  = \log\bracket{\frac{a \cdot 2^{p-1/2}}{x}}.
\end{equation}
By symmetry the negative bin $[-a, 0)$ gives the same integrand in $|x|$.
Therefore, for each marginal,
\begin{align}
  \int_{\mathcal{B}_0} f_{X_j}(x)
    \bigl|\log\bracket{\Delta_s(x)/\Delta(x)}\bigr|\,dx
  &\leq
  \sup_{t \in \mathcal{B}_0} f_{X_j}(t)
  \;\cdot\;
  2\int_0^{a} \log\bracket{\frac{a\cdot 2^{p-1/2}}{x}}dx.
\end{align}
The integral evaluates as
\begin{align}
  2\int_0^{a} \log\bracket{\frac{a\cdot 2^{p-1/2}}{x}}dx
  &= 2\int_0^{a}\Bigl[\bigl(p - \frac{1}{2}\bigr)
     + \log[a/x]\Bigr]dx \notag\\
  &= 2a\left(p - \frac{1}{2}\right)
     + \frac{2}{\ln 2}\int_0^{a}\ln[a/x]\,dx \notag\\
  &= 2a\left(p - \frac{1}{2}\right) + \frac{2a}{\ln 2}
  \;=\; 2a\left(p - \frac{1}{2} + \log e\right)
  \;=\; C_0,
\end{align}
where we used $\int_0^{a}\ln[a/x]\,dx = a$.
Summing over $j=1,\dots,d$ gives Eq.~\eqref{eq:eps_sp_general}.

When each $f_{X_j}$ has its mode at zero,
$\sup_{x\in\mathcal{B}_0} f_{X_j}(x) = f_{X_j}(0)$,
yielding Eq.~\eqref{eq:eps_sp_mode}.
Substituting $f_{X_j}(0)$ for $\mathcal{N}(0,\sigma_j^2)$ and
$t_\nu(0,\sigma_j)$ gives Eqs.~\eqref{eq:eps_sp_gauss}
and~\eqref{eq:eps_sp_student}.
\end{proof}
 
For candidate floating-point formats and identical marginals
($\sigma_j = \sigma$ for all $j$), Figure~\ref{fig:eps0_C0_vs_p}
shows $C_0$ and the per-dimension bound $\varepsilon_{0}/d$
as functions of the precision $p$ for several exponent widths $E$,
with $\sigma = 1$ and $d = 1$.
Gaussian marginals are shown as circles and
Student's $t_5$ marginals as squares; the two nearly overlap because
the ratio
$\Gamma\bigl(\frac{\nu+1}{2}\bigr)\sqrt{2/\nu}\big/\Gamma\bigl(\frac{\nu}{2}\bigr)$
is $O(1)$ for all $\nu \ge 1$.
By $E = 4$, $\varepsilon_0 \approx 0.16$ for $p = 24$. 

\begin{figure}[htbp]
  \centering
  \begin{subfigure}[t]{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{code/quantized_entropy_midpoint/C0_vs_p.pdf}
    \caption{$C_0$ vs.\ precision $p$.}
    \label{fig:C0_vs_p}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{code/quantized_entropy_midpoint/eps0_vs_p.pdf}
    \caption{$\varepsilon_{0}$ bound vs.\ precision $p$.}
    \label{fig:eps0_vs_p}
  \end{subfigure}
  \caption{Numerical scale of $C_0$ and $\varepsilon_{0}$ (Corollary~\ref{cor:eps_sp_bound}) for $d=1$, $\sigma=1$.
  Each curve corresponds to a different exponent width $E$.
  Circles denote Gaussian marginals; squares denote Student's $t_5$ marginals.}
  \label{fig:eps0_C0_vs_p}
\end{figure}

\FloatBarrier
% \subsubsection*{Approximation 3 -- $\mathbb{E}[\log[|x|/\sqrt{2}]]$}\label{app:FPN_app3}

% \begin{figure}[htbp]
%   \centering
%     \includegraphics[trim={1cm 0.0cm 16cm 0.85cm}, clip,width=0.5\textwidth]{code/quantized_entropy_midpoint/entropy_vs_mu_all_approx.pdf}
% \caption{\textit{Simulating approximation 3: }  The dependence of the entropy of a normally distributed floating-point number on its standard deviation $\sigma$ and mean $\mu$. Dashed lines show Approximation 3 from Eq.~\eqref{eq:three_approxes}, while solid lines show the exact entropy from Corollary~\ref{cor:gauss_fp_ent}.}\label{fig:fp_off_zero}
% \end{figure}

% We can show that Eq.~\eqref{eq:first_two_approx} approximates Eq.~\eqref{eq:three_approxes} in two cases. First, for a Gaussian distribution where its mean is significantly greater than its standard deviation, $\mu \gg \sigma$. Second, for a distribution $X \sim f_{X}(x,\epsilon)$ that approximates a Dirac delta function as $\epsilon \rightarrow 0$. 

% \textit{Non-zero mean Gaussian: }First, for a non-zero mean Gaussian, let $X = \mu + \epsilon$ where $\epsilon \sim \mathcal{N}(0, \sigma^2)$. Without loss of generality, assume $\mu > 0$ (the final result depends only on $|\mu|$). $\log\bracket{\abs{X/\sqrt{2}}}$ becomes\begin{align}
%     \log\left|\frac{X}{\sqrt{2}}\right| = \log\left|\frac{\mu + \epsilon}{\sqrt{2}}\right| 
%     = \log\left|\frac{\mu}{\sqrt{2}}\left(1 + \frac{\epsilon}{\mu}\right)\right| 
%     = \log\left|\frac{\mu}{\sqrt{2}}\right| + \log\left|1 + \frac{\epsilon}{\mu}\right|.\label{eq:split_x}
% \end{align}
% To control the second term, we can split according to the events
% \begin{equation}
%     A=\left\{\abs{\frac{\epsilon}{\mu}} \leq \frac{1}{2}\right\} = \left\{X \in \bracket{\frac{\mu}{2}, \frac{3\mu}{2}}\right\}, \qquad A^c= \left\{|\frac{\epsilon}{\mu}| > \frac{1}{2}\right\}.
% \end{equation}
% Events in $A^c$ are exponentially unlikely when $\mu\gg\sigma$, since $P(A^c)$ is equal to
% \begin{align}
%     \mathbb P(A^c)& =\int_{-\infty}^{-\mu/2} \frac{\exp[-t^2/2\sigma^2]}{\sigma \sqrt{2\pi}} dt + \int_{\mu/2}^{\infty} \frac{\exp[-t^2/2\sigma^2]}{\sigma\sqrt{2\pi}}\,dt  = 2 \int_{\mu/2}^{\infty} \frac{\exp[-t^2/2\sigma^2]}{\sigma\sqrt{2\pi}}\,dt. \\
%     &= 2\int_{\mu/2}^{\infty} \frac{\sigma}{t} \cdot
%        \frac{t}{\sigma^2} \cdot
%        \frac{\exp[-t^2/2\sigma^2]}{\sqrt{2\pi}}\,dt \leq \frac{4\sigma}{\mu} \int_{\mu/2}^{\infty}
%        \frac{t}{\sigma^2} \cdot
%        \frac{\exp[-t^2/2\sigma^2]}{\sqrt{2\pi}}\,dt \\
%     & = \frac{4\sigma}{\mu\sqrt{2\pi}}\left[-\exp\left[-\frac{t^2}{2\sigma^2}
%        \right]\right]_{\mu/2}^{\infty} = \frac{4\sigma}{\mu\sqrt{2\pi}}\,e^{-\mu^2/(8\sigma^2)}\label{eq:p_ac_bound}
% \end{align}
% meaning that for $\mu \gg \sigma$, $P(A^c)$ is small.

% By the law of total expectation,
% \begin{equation}\label{eq:total_expect}
%     \mathbb{E}\left[\log\left|1 + \frac{\epsilon}{\mu}\right|\right] = \mathbb{E}\left[\log\left|1 + \frac{\epsilon}{\mu}\right|\,\middle|\, A\right]P(A) + \mathbb{E}\left[\log\left|1 + \frac{\epsilon}{\mu}\right|\,\middle|\, A^c\right]P(A^c).
% \end{equation}
% For the first term, on $A$ we have $1+\epsilon/\mu > 0$, so the Mercator series converges:
% \begin{equation}
%     \log\left[1 + \frac{\epsilon}{\mu}\right] = \frac{1}{\ln[2]} \left( \frac{\epsilon}{\mu} - \frac{\epsilon^2}{2\mu^2} + O \left (\frac{\epsilon^3}{\mu^3}\right ) \right).
% \end{equation}
% Since $1+\epsilon/\mu > 0$ on $A$, the absolute value can be dropped. On $A = \{|\epsilon/\mu| \le 1/2\}$, the Mercator remainder satisfies $|\ln[1+x] - x + x^2/2| \le \frac{2}{3}|x|^3$ for $|x| \le 1/2$. Therefore,
% \begin{equation}
%     \E{\left|\ln\left(1+\frac{\epsilon}{\mu}\right) - \frac{\epsilon}{\mu} + \frac{\epsilon^2}{2\mu^2}\right| \Bigg|A} \le \frac{2}{3}\frac{\E{|\epsilon|^3|A}}{|\mu|^3} = O\left(\frac{\sigma^3}{\mu^3}\right).
% \end{equation}
% $\mathbb{E}[\epsilon \mid A] = 0$ since the distribution of $\epsilon$ is symmetric over the interval $\bracket{-\mu/2, \, \mu/2}$ and by the monotone convergence theorem as $\mu/\sigma \to \infty$,  $\mathbb{E}[\epsilon^2 \mid A] \to \sigma^2$. Thus,
% \begin{equation}
%     \mathbb{E}\left[\log\left|1 + \frac{\epsilon}{\mu}\right|\,\middle|\, A\right]P(A) = \frac{P(A)}{\ln[2]} \left( - \frac{\sigma^2}{2\mu^2} + O\left(\frac{\sigma^3}{|\mu|^3}\right) \right) \approx -\frac{\sigma^2}{2\mu^2 \ln[2]}.
% \end{equation}

% For the term pertaining to $A^c$, Lemma~\ref{lem:Ac-bound} shows that $\mathbb{E}\left[\left|\log\left|1 + \epsilon/\mu\right|\right|\,\middle|\, A^c\right]\mathbb{P}(A^c) \to 0$ as $\mu/\sigma \to \infty$, which means taking the expectation of Eq.~\eqref{eq:split_x} gives
% \begin{equation}
%     \mathbb{E} \left[\log\left|\frac{X}{\sqrt{2}}\right| \right] \approx \log\left|\frac{\mu}{\sqrt{2}}\right| - \frac{\sigma^2}{2\mu^2 \ln[2]}.
% \end{equation}
% As $\frac{\sigma^2}{2\mu^2 \ln[2]} \rightarrow 0$ as $\mu/\sigma \rightarrow \infty$, we see that the convolution integral can be approximated for $\mu \gg \sigma$ as 
% \begin{align}
%     G_{\mathcal{N}(\mu,\sigma^2)}(\mu)=\int^{\infty}_{-\infty} \frac{\exp(-\frac{(x-\mu)^2}{2\sigma^2})}{\sigma \sqrt{2\pi}} \, \log \bigg[\frac{|x|}{\sqrt{2}} \bigg] dx \approx \log\left[\frac{|\mu|}{\sqrt{2}}\right].
% \end{align}
% as shown in Fig.~\ref{fig:fp_off_zero}, which shows that the value of the convolution integral is insensitive to the value of $\sigma$ when $\mu \gg \sigma$. 

% \noindent This means for a non-zero mean Gaussian random variable, for $\mu \gg \sigma$, $\Ht_s(\Xfp) \approx \Ht_s^\mu(X_{fp})$, with
% \begin{equation}
%     \label{eq:int_entropy}
%     \Ht^\mu_s(\Xfp) \triangleq \frac{1}{2}\log[2\pi e \sigma^2] + (p-1) - \log\bracket{|\mu| / \sqrt{2}}.
% \end{equation}


% \begin{lemma}[Bound on the Mercator Series Remainder]\label{lem:mercator-remainder}
% For all $|x| \le \frac{1}{2}$,
% \begin{equation}
%   \abs{\ln[1+x] - x + \frac{x^2}{2}} \leq \frac{2}{3}\,|x|^3.
% \end{equation}
% \end{lemma}
 
% \begin{proof}
% The Mercator series gives
% \begin{equation}
%   \ln\bracket{1+x} \;=\; \sum_{k=1}^{\infty} \frac{(-1)^{k+1}\, x^k}{k},
%   \qquad |x| < 1,
% \end{equation}
% so the second-order remainder is
% \begin{equation}
%   R_2(x)
%   \triangleq \ln\bracket{1+x} - x + \frac{x^2}{2}
%   \;=\; \sum_{k=3}^{\infty} \frac{(-1)^{k+1}\, x^k}{k}.
% \end{equation}
% By the triangle inequality and using the inequality $1/k \le 1/3$ for every $k \ge 3$,
% \begin{equation}
%   |R_2(x)|
%   \;\le\; \sum_{k=3}^{\infty} \frac{|x|^k}{k}
%   \;\le\; \frac{1}{3} \sum_{k=3}^{\infty} |x|^k
%   \;=\; \frac{1}{3} \cdot \frac{|x|^3}{1 - |x|},
% \end{equation}
% where the last equality is the geometric series
% $\sum_{k=3}^{\infty} |x|^k = |x|^3 \sum_{j=0}^{\infty} |x|^j = |x|^3/(1-|x|)$,
% valid for $|x| < 1$.
% Since $|x| \le \frac{1}{2}$ implies $1 - |x| \ge \frac{1}{2}$, we obtain
% \begin{equation}
%   |R_2(x)|
%   \;\le\; \frac{|x|^3}{3 \paren{\frac{1}{2}}}
%   \;=\; \frac{2}{3}\,|x|^3.
% \end{equation}
% \end{proof}

% \begin{lemma}\label{lem:Ac-bound}
% Let $\epsilon \sim N(0,\sigma^2)$, $\mu \neq 0$, and $A = \{|\epsilon/\mu| \le \frac{1}{2}\}$.
% Then,
% \begin{equation}
%   \E{\abs{\ln\abs{1+\frac{\epsilon}{\mu}}}\,\, \Bigr|\,A^c}P(A^c)
%   \leq \,\paren{\frac{C_1\sigma}{|\mu|} + \frac{C_2|\mu|}{\sigma}}\, e^{-|\mu|^2/8\sigma^2}
% \end{equation}
% for some $C_1, C_2 > 0$.
% In particular, the bound decays faster than any polynomial in~$|\mu|/\sigma$.
% \end{lemma}

% \begin{proof}
% Write $Z = \epsilon/\sigma \sim N(0,1)$, so that $\epsilon/\mu = \sigma Z/\mu$
% (taking $\mu>0$ without loss of generality; the case $\mu<0$ is symmetric).
% Set $\delta \triangleq 1 + \epsilon/\mu = 1 + \sigma Z/\mu$ and split
% \begin{equation}
%   A^c = A_1^c \cup A_2^c, \qquad
%   A_1^c \triangleq \left\{\abs{\frac{\epsilon}{\mu}}>\frac{1}{2}\right\} \cap \left\{\abs{\delta}\ge \frac{1}{2}\right\},\qquad
%   A_2^c \triangleq \left\{\abs{\frac{\epsilon}{\mu}}>\frac{1}{2}\right\} \cap \left\{\abs{\delta} < \frac{1}{2}\right\}.
% \end{equation}

% \medskip
% \noindent\textit{Contribution of~$A_1^c$.}\enspace
% For $t \ge \frac{1}{2}$ we have $|\ln t| \le \ln 2 + t$
% (since $-\ln t \leq \ln 2$ when $t \geq \frac{1}{2}$,
% and $\ln t \le t$ when $t > 0$).  Hence on~$A_1^c$,
% \begin{equation}
%   |\ln{\abs{\delta}}| \;\le\; \ln 2 + |\delta|
%   \;\le\; \ln 2 + 1 + |\frac{\epsilon}{\mu}|
% \end{equation}
% almost surely.
% Therefore
% \begin{align}
% &\abs{\ln|\delta|}\indic{A_1^c} \;\le\; \paren{\ln 2 + 1 + |\frac{\epsilon}{\mu}|}\indic{A_1^c}\\
%   \implies &\E{\abs{\ln\bracket{|\delta|}}\indic{A_1^c}}
%   \;\le\; \E{\paren{\ln 2 + 1 + |\frac{\epsilon}{\mu}|}\indic{A_1^c}}\\
%   \implies &\E{\abs{\ln\bracket{|\delta|}}\indic{A_1^c}}
%   \;\le\; (1+\ln 2)\,P(A_1^c) + \E{\abs{\frac{\sigma Z}{\mu}}\indic{A_1^c}}\\
%     \implies &\E{\abs{\ln\bracket{|\delta|}}\indic{A_1^c}}
%   \;\le\; (1+\ln 2)\,P(A^c) \;+\;
%     \frac{\sigma}{\mu}\E{|Z|\,\mathbf{1}_{|Z|>\mu/2\sigma}},
% \end{align}
% since $A_1^c \subset A^c \implies P(A_1^c) \leq P(A^c)$ and $\indic{A_1^c} \leq \indic{A^c}$ almost surely.
% From Eq.~\eqref{eq:p_ac_bound}, the Gaussian tail bound gives
% $P(A^c) \leq \frac{4\sigma}{\mu\sqrt{2\pi}}\,e^{-\mu^2/(8\sigma^2)}$,
% and the truncated first moment evaluates to
% \begin{equation}
%   \mathbb{E}\bigl[|Z|\,\mathbf{1}_{|Z|>a}\bigr]
%   = \frac{2}{\sqrt{2\pi}}\int_a^\infty ze^{-\frac{z^2}{2}}dz = \frac{2}{\sqrt{2\pi}}\,e^{-a^2/2},
%   \qquad a = \frac{\mu}{2\sigma}.
% \end{equation}
% Since \begin{equation}
%     \E{\abs{\ln\abs{\delta}} \,|\, A_1^c}P(A_1^c) = \E{\abs{\ln\abs{\delta}}\indic{A_1^c}} \leq \paren{\ln 2 + \frac{3}{2}}\frac{4\sigma}{\mu\sqrt{2\pi}}\,e^{-\mu^2/(8\sigma^2)},
% \end{equation}
% the entire $A_1^c$~contribution is at most
% $\frac{C_1\sigma}{\mu}\,e^{-\mu^2/(8\sigma^2)}$ for some constant~$C_1$.

% \medskip
% \noindent\textit{Contribution of~$A_2^c$.}\enspace
% On the event $\{|\delta|<\frac{1}{2}\}$ we have
% $\epsilon/\mu \in (-\frac{3}{2},-\frac{1}{2})$,
% i.e.\ $Z \in (-\frac{3\mu}{2\sigma},-\frac{\mu}{2\sigma})$.
% The density of~$\delta$ at a point~$t$ is
% $\frac{\mu}{\sigma}f_Z\paren{\frac{\mu}{\sigma}(t-1)}$,
% where $f_Z$ is the standard normal density.
% For $\abs{t}<\frac{1}{2}$ we have $(t-1)^2 \ge \frac{1}{4}$, giving the
% uniform density bound
% \begin{equation}
%   \frac{\mu}{\sigma}f_Z\paren{\frac{\mu}{\sigma}(t-1)}
%   = \frac{\mu}{\sigma\sqrt{2\pi}}e^{-\frac{\mu^2(t-1)^2}{2\sigma^2}}
%   \leq \frac{\mu}{\sigma\sqrt{2\pi}}\,e^{-\frac{\mu^2}{8\sigma^2}}.
% \end{equation}
% Since $\abs{\delta} < \frac{1}{2}$ almost surely implies $\abs{\frac{\epsilon}{\mu}}>\frac{1}{2}$ almost surely, we have $A_2^c = \{\abs{\delta} < \frac{1}{2}\}$ and
% \begin{equation}
%   \E{\abs{\ln\abs{\delta}}\,\indic{|\delta|<1/2}}
%   = \int_{-1/2}^{1/2}\frac{\mu}{\sigma}f_Z\paren{\frac{\mu}{\sigma}(t-1)}\abs{\ln\abs{t}}dt
%   \leq
%   \frac{\mu}{\sigma\sqrt{2\pi}}\,e^{-\frac{\mu^2}{8\sigma^2}}
%   \int_{-1/2}^{1/2} |\ln\abs{t}\,|\,dt.
% \end{equation}
% The integral evaluates to
% $-2\int_0^{1/2}\ln\bracket{t}\,dt = -2\bracket{t\ln t -t}\Bigr|_0^{1/2}
% = \ln 2 + 1$,
% so the $A_2^c$~contribution is at most
% $\frac{C_2\mu}{\sigma}\,e^{-\frac{\mu^2}{8\sigma^2}}$ for some constant $C_2$.

% \medskip
% \noindent\textit{Combining both contributions.}\enspace
% Adding both contributions yields
% \begin{equation}
%   \E{\abs{\ln\abs{1+\frac{\epsilon}{\mu}}}\,\mathbf{1}_{A^c}}
%   \;\le\; \paren{\frac{C_1\sigma}{\mu} + \frac{C_2\mu}{\sigma}} e^{-\frac{\mu^2}{8\sigma^2}}
% \end{equation}
% which decays faster than any polynomial in~$|\mu|/\sigma$.
% \end{proof}

% \textit{Approximating delta distribution: } Next, we can show the same result for a function which approximates a delta function as $\varepsilon \rightarrow 0$, provided $\mu \neq 0$. For a random variable $X$ where $f_X(x-\mu; \varepsilon) \rightarrow \delta (x-\mu)$ as $\varepsilon \rightarrow 0$ with $\mu \neq 0$, Eq.~\eqref{eq:G_int_non_gauss} becomes
% \begin{equation}
%     G_{f_X}(\mu) \triangleq \int^{\infty}_{-\infty} f_X(x-\mu; \epsilon) \log \bigg[\frac{|x|}{\sqrt{2}} \bigg] dx.
% \end{equation}
% As $\epsilon \rightarrow 0$, for any $\mu \neq 0$ such that $\log[|x| / \sqrt{2}]$ is continuous,
% \begin{align*}
%     G_{f_X}(\mu) & \approx \int^{\infty}_{-\infty} \delta(x-\mu) \log \bigg[\frac{|x|}{\sqrt{2}} \bigg] dx \\
%     & = \log \bigg[\frac{|\mu|}{\sqrt{2}} \bigg].
% \end{align*}
% Thus for any distribution, which may be non-Gaussian, if it approaches $\delta(\cdot)$ as a parameter $\epsilon$ which defines it approaches 0 and $\mu \neq 0$, in the limit of $\epsilon \rightarrow 0$ the integral term satisfies $G_{f_X}(\mu) \approx \log[|\mu|/\sqrt{2}]$, giving $\Ht_s(X_{fp}) \approx \Ht_s^\mu(X_{fp})$, where
% \begin{equation}
%     \Ht^\mu_s(\Xfp) \triangleq h(X) + (p-1) - \log\bracket{|\mu| / \sqrt{2}}.
% \end{equation}

% \FloatBarrier
\pagebreak


==> appendices/avg_sum_cost.tex <==
\section{Landauer Cost of Averaging and Summing}\label{sec:avg_sum}
An even simpler prediction algorithm than linear regression is the average. Let the input to this algorithm be $X_1,\dots, X_n \iid f$, where $\E{X_i} = \mu$ and $\mathrm{var}\paren{X_i} = \sigma^2$. The differential entropy of the input is $h(X_1, \dots, X_n) = nh(X_1)$.

If $f$ is not Gaussian, for sufficiently large $n$, central limit theorem can be invoked to show that $\frac{1}{n}\sum\limits_{i = 1}^n X_i \Rightarrow \gauss{\mu}{\frac{\sigma^2}{n}}$ as $n \rightarrow \infty$. So the differential entropy of the final distribution is $h(\frac{1}{n}\sum\limits_{i = 1}^n X_i) \approx \frac{1}{2}\log\bracket{2\pi e \frac{\sigma^2}{n}}$. When $f_{X_i}$ is Gaussian, this is true even for small $n$.

For the case when $ \forall i, f_{X_i} \sim \gauss{0}{1}$ and the random variable are encoded in floating-point numbers with precision $p$, the discrete entropy difference is
\begin{align}
    \Delta H = n\Ht^0_{s}(p) - \Ht^0_{s}(p) = (n-1)\Ht^0_{s} \approx (n-1)(p + 2.46) \text{ bits,}\label{eq:landauer_avg}
\end{align}
where $\Ht^0_{s}(p)$ is derived in Section~\ref{sec:fpn}. Notice that Eq.~\eqref{eq:landauer_avg} is dominated by the number of inputs. As stressed in Section~\ref{sec:fpn}, $\Ht^0_{s}(p)$ does not depend on the variance of the random variable. This means that for zero-mean Gaussian random variables, the Landauer cost of averaging $\frac{1}{n}\sum\limits_{i = 1}^n X_i$ and summing $\sum\limits_{i = 1}^n X_i$ is equivalent, since $\sum\limits_{i = 1}^n X_i \sim \gauss{0}{n\sigma^2}$.




\FloatBarrier
\pagebreak


==> appendices/diff_entropy_z.tex <==
\section{Computing the Differential Entropy of Z}\label{sec:compute_h_z}

\begin{lemma}\label{lem:diff_ent_Ex}
    Under the hypotheses of Lemma~\ref{lem:compute_f_z}, let $\psi(x) \triangleq \frac{d}{dx}\ln{\Gamma(x)} = \frac{\Gamma^\prime(x)}{\Gamma(x)}$ be the digamma function. The differential entropy of $Z$ is
\begin{align}
    \label{eq:diff_ent_Ex}
    h(Z) &= \log\bracket{e}\paren{\ln\bracket{\frac{\sigxi}{\sigx}} - \ln{\paren{\frac{\Gamma\paren{\frac{n+1}{2}}}{\sqrt{\pi}\Gamma\paren{\frac{n}{2}}}}} + \frac{n + 1}{2}\bracket{\psi\paren{\frac{n+1}{2}} - \psi\paren{\frac{n}{2}}}}.
\end{align}
\end{lemma}


\begin{proof}[Proof of Lemma~\ref{lem:diff_ent_Ex}]
    Using the distribution derived in Lemma~\ref{lem:compute_f_z}, the differential entropy of $Z$ is
\begin{align}
    &\frac{1}{\log\bracket{e}}h(Z) = -\int\limits_{-\infty}^\infty f_Z(z)\ln{f_Z(z)}dz\\
     &= -\int\limits_{-\infty}^\infty \paren{\sqrt{\frac{1}{\pi\paren{\sigx^2}^n\sigxi^2}}\frac{\Gamma\paren{\frac{n+1}{2}}}{\Gamma\paren{\frac{n}{2}}}\paren{\frac{\sigx^2\sigxi^2}{\sigx^2z^2 + \sigxi^2}}^{\frac{n + 1}{2}}}\\
     &\times\ln{\paren{\sqrt{\frac{1}{\pi\paren{\sigx^2}^n\sigxi^2}}\frac{\Gamma\paren{\frac{n+1}{2}}}{\Gamma\paren{\frac{n}{2}}}\paren{\frac{\sigx^2\sigxi^2}{\sigx^2z^2 + \sigxi^2}}^{\frac{n + 1}{2}}}}dz\\
     &= -\int\limits_{-\infty}^\infty \paren{\sqrt{\frac{1}{\pi\paren{\sigx^2}^n\sigxi^2}}\frac{\Gamma\paren{\frac{n+1}{2}}}{\Gamma\paren{\frac{n}{2}}}\paren{\frac{\sigx^2\sigxi^2}{\sigx^2z^2 + \sigxi^2}}^{\frac{n + 1}{2}}}\nonumber\\
     &\bracket{ \ln{\paren{\sqrt{\frac{1}{\pi\paren{\sigx^2}^n\sigxi^2}}\frac{\Gamma\paren{\frac{n+1}{2}}}{\Gamma\paren{\frac{n}{2}}}\paren{\sigxi^2}^{\frac{n + 1}{2}}}}- \frac{n + 1}{2}\ln\bracket{z^2 + \frac{\sigxi^2}{\sigx^2}}}dz\\
     &= -\sqrt{\frac{1}{\pi\paren{\sigx^2}^n\sigxi^2}}\frac{\Gamma\paren{\frac{n+1}{2}}}{\Gamma\paren{\frac{n}{2}}} \ln{\paren{\sqrt{\frac{1}{\pi\paren{\sigx^2}^n\sigxi^2}}\frac{\Gamma\paren{\frac{n+1}{2}}}{\Gamma\paren{\frac{n}{2}}}\paren{\sigxi^2}^{\frac{n + 1}{2}}}}\int\limits_{-\infty}^\infty \paren{\frac{\sigx^2\sigxi^2}{\sigx^2z^2 + \sigxi^2}}^{\frac{n + 1}{2}} dz\\
     &+ \frac{n + 1}{2}\sqrt{\frac{1}{\pi\paren{\sigx^2}^n\sigxi^2}}\frac{\Gamma\paren{\frac{n+1}{2}}}{\Gamma\paren{\frac{n}{2}}}\int\limits_{-\infty}^\infty \paren{\frac{\sigx^2\sigxi^2}{\sigx^2z^2 + \sigxi^2}}^{\frac{n + 1}{2}}\ln\bracket{z^2 + \frac{\sigxi^2}{\sigx^2}}dz\\
     &= - \ln{\paren{\sqrt{\frac{1}{\pi\paren{\sigx^2}^n\sigxi^2}}\frac{\Gamma\paren{\frac{n+1}{2}}}{\Gamma\paren{\frac{n}{2}}}\paren{\sigxi^2}^{\frac{n + 1}{2}}}}\nonumber\\
     &+ \frac{n + 1}{2}\sqrt{\frac{1}{\pi\paren{\sigx^2}^n\sigxi^2}}\frac{\Gamma\paren{\frac{n+1}{2}}}{\Gamma\paren{\frac{n}{2}}}\int\limits_{-\infty}^\infty \paren{\frac{\sigx^2\sigxi^2}{\sigx^2z^2 + \sigxi^2}}^{\frac{n + 1}{2}}\ln\bracket{z^2 + \frac{\sigxi^2}{\sigx^2}}dz\label{eq:normalized}
\end{align}

The first term in Eq.~\eqref{eq:normalized} is due to $f_Z(z)$ being a probability density function.

Just solving for $\int\limits_{-\infty}^\infty \paren{\frac{\sigx^2\sigxi^2}{\sigx^2z^2 + \sigxi^2}}^{\frac{n + 1}{2}}\ln\bracket{z^2 + \frac{\sigxi^2}{\sigx^2}}dz$, let $\psi(x) \triangleq \frac{d}{dx}\ln{\Gamma(x)} = \frac{\Gamma^\prime(x)}{\Gamma(x)}$. Using the change of variables $\theta = \tan^{-1}(\frac{\sigx z}{\sigxi})$,


\begin{align}
    &\int\limits_{-\infty}^\infty \paren{\frac{\sigx^2\sigxi^2}{\sigx^2z^2 + \sigxi^2}}^{\frac{n + 1}{2}}\ln\bracket{z^2 + \frac{\sigxi^2}{\sigx^2}}dz = \sigx^n\sigxi\int\limits_{-\frac{\pi}{2}}^\frac{\pi}{2} \paren{\frac{1}{\sec^2{\theta}}}^{\frac{n - 1}{2}}\ln\bracket{\frac{\sigxi^2}{\sigx^2}\sec^2\theta}d\theta\\
    &=  \sigx^n\sigxi\bracket{\int\limits_{-\frac{\pi}{2}}^\frac{\pi}{2} \paren{\frac{1}{\sec^2{\theta}}}^{\frac{n-1}{2}}\ln\bracket{\sec^2\theta}d\theta + \ln\bracket{\frac{\sigxi^2}{\sigx^2}}\int\limits_{-\frac{\pi}{2}}^\frac{\pi}{2} \paren{\frac{1}{\sec^2{\theta}}}^{\frac{n-1}{2}}d\theta}\\
    &=  \sigx^n\sigxi\bracket{\frac{\sqrt{\pi}\Gamma\paren{\frac{n}{2}}\paren{\psi\paren{\frac{n+1}{2}} - \psi\paren{\frac{n}{2}}}}{\Gamma\paren{\frac{n+1}{2}}}  + \frac{\ln\bracket{\frac{\sigxi^2}{\sigx^2}}\sqrt{\pi}\Gamma\paren{\frac{n}{2}}  }{\Gamma\paren{\frac{n+1}{2}}}}\\
    &= \frac{ \sigx^n\sigxi\sqrt{\pi}\Gamma\paren{\frac{n}{2}}}{\Gamma\paren{\frac{n+1}{2}}}\bracket{\psi\paren{\frac{n+1}{2}} - \psi\paren{\frac{n}{2}} + \ln\bracket{\frac{\sigxi^2}{\sigx^2}}}.
\end{align}

Now returning to the computation of $h(Z)$, we have
\begin{align}
    \frac{1}{\log\bracket{e}}h(Z) &= - \ln{\paren{\sqrt{\frac{1}{\pi\paren{\sigx^2}^n\sigxi^2}}\frac{\Gamma\paren{\frac{n+1}{2}}}{\Gamma\paren{\frac{n}{2}}}\paren{\sigxi^2}^{\frac{n + 1}{2}}}}\nonumber\\ 
    &+ \frac{n + 1}{2}\bracket{\psi\paren{\frac{n+1}{2}} - \psi\paren{\frac{n}{2}} + \ln\bracket{\frac{\sigxi^2}{\sigx^2}}}\\
    &= - \ln{\paren{\frac{\sigxi^n}{\sqrt{\pi}\sigx^n}\frac{\Gamma\paren{\frac{n+1}{2}}}{\Gamma\paren{\frac{n}{2}}}}} + \frac{n + 1}{2}\bracket{\psi\paren{\frac{n+1}{2}} - \psi\paren{\frac{n}{2}} + \ln\bracket{\frac{\sigxi^2}{\sigx^2}}}\\
    &= \ln\bracket{\frac{\sigxi}{\sigx}} - \ln{\paren{\frac{\Gamma\paren{\frac{n+1}{2}}}{\sqrt{\pi}\Gamma\paren{\frac{n}{2}}}}} + \frac{n + 1}{2}\bracket{\psi\paren{\frac{n+1}{2}} - \psi\paren{\frac{n}{2}}}.
\end{align}
\end{proof}

\begin{figure}[htbp]
  \centering
  \begin{subfigure}{0.4\textwidth}
    \centering
    \includegraphics[width=\linewidth]{code/quantized_entropy_midpoint/exact_lr/H_wh_fp_vs_n.pdf}
    \caption{}
    \label{fig:H_fp_wh_exact}
  \end{subfigure}
  \begin{subfigure}{0.4\textwidth}
    \centering
    \includegraphics[width=\linewidth]{code/quantized_entropy_midpoint/exact_lr/landauer_cost_per_n_vs_n.pdf}
    \caption{}
    \label{fig:Ex_dH_exact}
  \end{subfigure}\hfill
  \caption{\textit{The Landauer cost for exact zero-intercept simple linear regression.} Input and output states are floating-point numbers with $p = 4$ and $E=4$. The candidate values of the $SNR = \frac{w^2\sigx^2}{\sigxi^2}$ are $0.062$, $0.25$, $1$, $4$, and $25$. (\ref{fig:H_fp_wh_exact}) The output model entropy, and its dependence on the data size $n$ and ground truth $w$. (\ref{fig:Ex_dH_exact}) The entropy difference for various values of SNR and a range of $n$.}
  \label{fig:exact_lr_ent}
\end{figure}



\FloatBarrier
\pagebreak


==> appendices/extended_kostina_proofs.tex <==
\section{Extending Theorem's in Kostina Paper to Float Setting}

\thinkabout{Midpoint quantization is dealing with L1 norm nearest neighbors instead of L2 norm. Noting that this product lattice structure, where each coordinate is quantized independently, is inefficient (check \cite[section 4.e]{GrayNeuhoff1998Quantization}). In 1D, all of the $L^p$ norms are just the absolute value.}

\begin{theorem}[Kostina, Theorem 8, bound on $\relent{X}{X_\mathcal{C}}$. Particularized to scalar case, and extended to nonuniform bins]
Let $X$ be a random variable with $h(X) > -\infty$ and $v$-regular density. Let $q: \R{} \mapsto \R{}$ be a quantizer with cells $\{\mathcal{V}_c\}$. Then the information random variable and the entropy at the output of the lattice quantizer can be bounded as
\begin{align}
\imath(q_{\mathcal{C}}(x)) &\leq \log \frac{1}{f_X(x)} - \log \Delta(x) + \Delta(x) v_{\mathcal{C}}(x) \log e, \label{eq:info_bound} \\
H(q_{\mathcal{C}}(X)) &\leq h(X) - \E{\log \Delta(X)} + \E{\Delta(X)v_{\mathcal{C}}(X)} \log e, \label{eq:entropy_bound}
\end{align}
where for each representable value $c$, $r_{c} = \max\limits_{x \in \mathcal{V}_{c}}\norm{x - c}{2}$ is the lattice covering radius, and $v_{\mathcal{C}}(x)$ is given by
\begin{equation}
v_{\mathcal{C}}(x) = \max_{u \in \mathcal{V}_{\mathcal{C}}(q_{\mathcal{C}}(x))} v(u).
\end{equation}
% Furthermore, if $v(x) = v(\norm{x}{2})$ is convex and nondecreasing, then \eqref{eq:info_bound} and \eqref{eq:entropy_bound} can be strengthened by replacing the above with
% \begin{equation}
% v_{\mathcal{C}}(x) = \frac{1}{2} v(\norm{x}{2}) + \frac{1}{2} v(\norm{x}{2} + 2r_{\mathcal{C}}),
% \end{equation}
% and if $v(x) = c_1 \norm{x}{2} + c_0$, then this particularizes as
% \begin{equation}
% v_{\mathcal{C}}(x) = c_1 \norm{x}{2} + c_1 r_{\mathcal{C}} + c_0.
% \end{equation}
\end{theorem}

\begin{proof}
Observe that,
\begin{align}
|\log f_X(a) - \log f_X(b)|
&= \left| \int_0^1 \innprod{\nabla \log f_X(ta + (1-t)b)}{a - b} \, dt \right| \\
&\leq \norm{a - b}{2} \log e \int_0^1 v(ta + (1-t)b) \, dt\label{eq:cauchyschwarz} \\
&\leq \max_{0 \leq t \leq 1} v(ta + (1-t)b) \norm{a - b}{2} \log e,\label{eq:logbound}
\end{align}
where \eqref{eq:cauchyschwarz} holds by Cauchy-Schwarz inequality. 
\thinkabout{Since $\norm{x}{2}\leq \norm{x}{1}$ we could have a looser bound wrt the $\norm{\cdot}{1}$ norm.}

For each $c \in \mathcal{C}$, $f_{X_c}(c - u_c) = \frac{P\{X \in \mathcal{V}_\mathcal{C}(c)\}}{\Delta(c)}$. Let $U_c \sim \unif{- \frac{\Delta(c)}{2}}{\frac{\Delta(c)}{2}}$, for all $u \in [- \frac{\Delta(c)}{2}, \frac{\Delta(c)}{2}]$, we have 
\begin{align}
    f_{X_c}(c - u) = \E{f_X(c + U_c)},
\end{align}
so by the MVT, there exists a $u_c \in  [- \frac{\Delta(c)}{2}, \frac{\Delta(c)}{2}]$ where
\begin{equation}
f_X(c - u_c) = f_{X_c}(c - u).\label{eq:mvt}
\end{equation}


Using \eqref{eq:mvt} and \eqref{eq:logbound} with $a=x$ and $b =q_{\mathcal{C}}(x) - u_c$, we evaluate the information in $q_{\mathcal{C}}(x)$ as
\begin{align}
\imath(q_{\mathcal{C}}(x))
&= \log \frac{1}{f_{X_{\mathcal{C}}}(x)} - \log \Delta(x) \\
&= \log \frac{1}{f_X(x)} - \log \Delta(x) + \log \frac{f_X(x)}{f_X(q_{\mathcal{C}}(x) - u_c)} \\
&\leq \log \frac{1}{f_X(x)} - \log \Delta(x)\nonumber\\ & + \max_{0 \leq t \leq 1} v(tx + (1-t)(q_{\mathcal{C}}(x) - u_c)) \norm{x - \paren{q_{\mathcal{C}}(x) - u_c}}{2} \log e\label{eq:preconvexity}\\
&\leq \log \frac{1}{f_X(x)} - \log \Delta(x)\nonumber\\ & + v_{\mathcal{C}}(x)\paren{\norm{x - q_{\mathcal{C}}(x)}{2} + \norm{u_c}{2}} \log e\label{eq:convexityrequired}\\
&\leq \log \frac{1}{f_X(x)} - \log \Delta(x) + \Delta(x)v_{\mathcal{C}}(x) \log e\\
&= \log \frac{1}{f_X(x)} - \log \Delta(x)+ 2r_{c}(x) v_{\mathcal{C}}(x) \log e,
\end{align}
which is equivalent to \eqref{eq:info_bound}, and \eqref{eq:entropy_bound} is immediate upon taking an expectation of \eqref{eq:info_bound}.



\thinkabout{There are nuances that come with higher dimension. In the above proof, going from \eqref{eq:preconvexity} to \eqref{eq:convexityrequired} requires convexity of each cell, and this might not hold for midpoint quantization due to the L1 nearest neighbors as opposed to L2. Need to check if the proof will still go through. Convexity of each cell hold trivially for the scalar case. For the scalar case $r_\mathcal{C} = \Delta/2$, but for a cubic lattice in $\R{n}$, $r_\mathcal{C} = 1/2\sqrt{\sum_{i = 1}^{n}\Delta^2} = \frac{\sqrt{n}\Delta}{2}$. A spherical lattice has a different scaling. $\rho_\mathcal{C}$ in the Kostina paper quantifies these different scalings.}



% If $v(x) = v(\norm{x}{2})$, convex and nondecreasing, we strengthen (128) by applying Jensen's inequality to (127):
% \begin{align}
% |\log f_X(a) - \log f_X(b)|
% &\leq \frac{\log e}{2} (v(\norm{a}{2}) + v(\norm{b}{2})) \norm{a - b}{2} \\
% &\leq \log e (v(\norm{a}{2}) + v(\norm{a}{2} + 2r_{\mathcal{C}})) r_{\mathcal{C}},
% \end{align}
% where to get (133) we used the triangle inequality, the assumption that $v$ is nondecreasing, and the fact that $\norm{a - b}{2} \leq 2r_{\mathcal{C}}$ for $a$ and $b$ from the same quantization cell. Modifying (131) accordingly results in a strengthening of (121) and (122) with $v_{\mathcal{C}}$ in (124).
\end{proof}

==> appendices/gaussian_approx.tex <==
\section{Applying approximations to the Gaussian case}\label{app:FPN_app_gauss}

Here the theorems for the floating point entropy of Gaussian random variables are reviewed. See Figure~\ref{fig:fp_exponents} for a directly computed histogram of exponent values. Directly computing the entropy of the histograms returns a discrete entropy of $\sim 2.54$ bits, which is close to the offset factor above the mantissa contribution $p$ in $\Ht^0_s(p) \approx p + 2.46$ bits. Since bin sizes are fairly large with respect to the underlying distribution of exponents, this divergence likely can be explained by quantization noise.

\begin{figure}[htbp]
  \centering
    \includegraphics[width=0.36\linewidth]{fpn/exponents (2).pdf}
\caption{\textit{Histogram of exponent values for a normally distributed random variable.} The distribution of exponent states for $X \sim \mathcal{N}(0,\sigma^2)$. From left to right, the distributions plotted have $\sigma = \{10^{-3}, 10^0, 10^3 \}$. All three have a discrete entropy $H(\log[X]) \approx 2.54$ bits. These distributions conform well to observational data in \cite{bordawekar2022efloatentropycodedfloatingpoint, hao_neuzip_2024}.}
    \label{fig:fp_exponents}
\end{figure}

\begin{theorem}[Approximating the entropy of a mean-zero univariate gaussian]
    \label{thm:single_gaussian}
    The discrete entropy of a zero-mean normally distributed continuous random variable $X \sim \mathcal{N}(0, \sigma_x^2)$ as represented on a floating-point number, with the approximations specified by Eq.~\eqref{eq:diff_approx} and~\eqref{eq:step_approx} applied, is a constant specified by the floating point number's precision, $p$.
    \begin{equation}
        \tilde H_s(X_{fp}) = (p-1) + \frac{1}{2} \log[2 \pi e] + 1 + \frac{\gamma_e}{2\ln[2]}
    \end{equation}
    
\end{theorem}
\begin{proof}
    Let $X \sim \mathcal{N}(0, \sigma_x^2)$.
    \begin{equation}
    \begin{aligned}
    \label{eq:1d-0m-fp}
        \Ht_{s}(\Xfp) &\triangleq h(X) - \E{\log[\Delta_s(x)]} \\
        &= \frac{1}{2}\log[2\pi e \sigma^2_x] - \int^{\infty}_{-\infty} \frac{\exp(-\frac{x^2}{2\sigma_x^2})}{\sigma_x \sqrt{2\pi}} \log [\Delta_s(x)] \, dx  \\
        &= \frac{1}{2}\log[2\pi e \sigma^2_x] - \int^{\infty}_{-\infty} \frac{\exp(-\frac{x^2}{2\sigma_x^2})}{\sigma_x \sqrt{2\pi}} (\log[|x|/\sqrt{2}] - (p - 1)) \, dx \\
        & = \frac{1}{2}\log[2\pi e \sigma^2_x] + (p - 1) - 2\int^{\infty}_0 \frac{\exp(-\frac{x^2}{2\sigma_x^2})}{\sigma_x \sqrt{2\pi}} \log[x/\sqrt{2}] \, dx\\
        & = \frac{1}{2}\log[2\pi e \sigma^2_x] + (p-1) + \bigg(1 + \frac{\gamma_e}{2\ln[2]} -\frac{1}{2} \log[\sigma^2_x] \bigg)\\
        & = (p-1) + \frac{1}{2} \log[2 \pi e] + 1 + \frac{\gamma_e}{2\ln[2]}\\
        & = p + \frac{1}{2} \log[2 \pi e] + \frac{\gamma_e}{2\ln[2]}.
    \end{aligned}
\end{equation}
\end{proof}

\begin{theorem}
    \label{thm:double_gaussian}
    Let $X \sim \mathcal{N}(0,\sigma_x^2)$, $\Xi \sim \mathcal{N}(0,\sigma_\xi^2)$, $w \in \mathbb{R}$, and $Y = wX + \Xi$. The approximate joint discrete entropy of $(\Xfp, \Yfp)$ is,
\begin{equation*}
    \Ht_s(\Xfp, \Yfp) = 2 \Ht^0_s(p)-\frac{1}{2} \log \bigg [ 1+\frac{\sigma_x^2 w^2}{\sigma_\xi^2} \bigg].
\end{equation*}
\end{theorem}
\begin{proof}
\begin{equation}
\label{eq:approx_joint_ent_SNR_start}
    \begin{aligned}
        \Ht_s(\Xfp, \Yfp) &\triangleq h(X, Y) - \iint_{-\infty}^\infty f_{XY}(x,y) ( \log[\Delta_s(x)] + \log[\Delta_s(y)])dxdy \\
        = h& (X)  + h(\Xi) - \iint_{-\infty}^\infty f_{XY}(x,y)  \log[\Delta_s(x)] dxdy - \iint_{-\infty}^\infty f_{XY}(x,y)\log[\Delta_s(y)]dxdy \\
        = \frac{1}{2}&\log[2\pi e \sigma_x^2] + \frac{1}{2}\log[2\pi e \sigma_\xi^2] - \int_{-\infty}^\infty f_{X}(x)  \log[\Delta_s(x)] dx - \int_{-\infty}^\infty f_{Y}(y)\log[\Delta_s(y)]dy.
    \end{aligned}
\end{equation}
where $h(X,Y) = h(X) + h(\Xi)$ is because $X$ is independent from $\Xi$ and $(X,\Xi) \mapsto (X,Y)$ is an invertible linear transformation with Jacobian 1. The expressions follow directly from the differential entropy of a normal distribution \cite{CoverThomas}. In the last line, $f_X(x)$ and $f_Y(y)$ are the marginal distributions over $f_{XY}(x,y)$,
\begin{equation}
    f_X(x) = \int_{-\infty}^\infty f_{XY}(x,y) \, dy\text{,  }f_Y(y) = \int_{-\infty}^\infty f_{XY}(x,y) \, dx,
\end{equation}
where from Eq.~\eqref{eq:initial_dist}
\begin{equation}
    f_X(x) =
\frac{1}{\sqrt{2\pi\sigma_x^2}}
\exp\left(-\frac{x^2}{2\sigma_x^2}\right)\text{,  } f_Y(y) =
\frac{1}{\sqrt{2\pi(\sigma_\xi^2+w^2\sigma_x^2)}}
\exp\left(-\frac{y^2}{2(\sigma_\xi^2+w^2\sigma_x^2)}\right).
\end{equation}
Applying the same steps as in Theorem~\ref{thm:single_gaussian} to evaluate the bin terms, we obtain
\begin{equation}
    \int_{-\infty}^{\infty} f_X(x)\,\log\bracket{\Delta_s(x)}\,dx
\approx
-\left(p+\frac{\gamma_e}{2\ln 2}\right)
+\frac{1}{2}\log \sigma_x^2,
\end{equation}

\begin{equation}
    \int_{-\infty}^{\infty} f_Y(y)\,\log\bracket{\Delta_s (y)}\,dy
    \approx
    -\left(p+\frac{\gamma_e}{2\ln 2}\right)
    +\frac{1}{2}\log\bracket{\sigma_\xi^2+w^2\sigma_x^2}.
\end{equation}
Plugging these back into the original expression, we obtain
\begin{equation}
    \label{eq:approx_joint_ent_SNR_app}
    \begin{aligned}
        \Ht_s(\Xfp, \Yfp) &= \frac{1}{2}\log[2\pi e \sigma_x^2] + \frac{1}{2}\log[2\pi e \sigma_\xi^2] + p+\frac{\gamma_e}{2\ln 2} - \frac{1}{2}\log \sigma_x^2\\
        & + p + \frac{\gamma_e}{2\ln[2]} - \frac{1}{2} \log[\sigma^2_\xi + \sigma_x^2 w^2].
    \end{aligned}
\end{equation}
Using the definition $H^0_s(p)$ from definition Eq.~\eqref{eq:single_mean_0} and Theorem~\ref{thm:single_gaussian}, we can obtain a clean final expression,
\begin{equation}
    \Ht_s(\Xfp, \Yfp) = 2 \Ht^0_s(p)-\frac{1}{2} \log \bigg [ 1+\frac{\sigma_x^2 w^2}{\sigma_\xi^2} \bigg]
\end{equation}
\end{proof}

















==> appendices/mismatch_cost_app.tex <==
\section{Mismatch Cost}
\label{app:mmc}

\subsubsection{Defining $\Delta S_{env}$ and $\Delta S_{tot}$ with a Continuous Time Markov Chain}

One general way to model such a time dependence is via a continuous time Markov chain (CTMC) based on transition rates between states of the joint computational system \cite{Wolpert2019, Manzano2024, KolchinskyWolpert2021, Owen_2019, esposito2010}. In this case, the dynamics of the computational system are fixed by a time varying matrix $W_{x_c,x_c'}(t)$, which defines the rate of transitions between states $x_c, x_c'\in \mathcal{X}_c$ at time $t$ \cite{Wolpert2019, KolchinskyWolpert2021}. 
While running an algorithm, the computational system evolves according to
\begin{equation}
    \label{eq:CTMC}
    \frac{d}{dt} p(x_c,t) = \sum_{x'_c \in \mathcal{X}_c} W_{x_c;x_c'}(t) p(x_c',t).
\end{equation}
For these dynamics, \cite{esposito2010} shows
\begin{equation}
    \Delta S_{sys} = -k_B \ln[2] \int^{t_f}_0 \sum_{x_c,x_c' \in \mathcal{X}_c} W_{x_c,x_c'}(t)p(x_c', t) \log \bigg[ \frac{p(x_c,t)}{p(x_c',t)} \bigg]dt,
\end{equation}
\begin{equation}
    \label{eq:s_env}
    \Delta S_{env} = - k_B \ln[2] \int^{t_f}_0\sum_{x_c,x_c'\in \mathcal{X}_c} W_{x_c,x_c'}(t) p(x_c', t) \log \bigg[ \frac{W_{x_c',x_c}(t)}{W_{x_c,x_c'}(t)} \bigg] dt,
\end{equation}
\begin{equation}
    \Delta S_{tot} = k_B \ln[2] \int^{t_f}_0\sum_{x_c,x_c'\in \mathcal{X}_c} W_{x_c,x_c'}(t) p(x_c', t) \log \bigg[ \frac{W_{x_c,x_c'}(t)p(x_c',t)}{W_{x_c',x_c}(t) p(x_c,t)} \bigg] dt.
\end{equation}
If the transition rates $W_{x_c,x_c'}$ satisfy $\ln[W_{x_c,x_c'}/W_{x_c',x_c}] = (E(x_c') - E(x_c))/(k_BT)$, where $E(x_c)$ is an energy function over computational states, then we can say the average heat is given by $Q = T \Delta S_{env}$ \cite[p.30]{Wolpert2019} \cite{Seifert_2012}. This implies that the average heat output, fixed by Eqs.~\eqref{eq:CTMC},~\eqref{eq:s_env} is given by $Q = T(-\Delta S_{sys} + \Delta S_{tot}) = \Delta E_{min} +T\Delta S_{tot}$. 












Let $\compsimplex$ denote the probability simplex associated with the computational state space $\mathcal{X}_c$. We can think of the computation which takes us from $p_1 \in \compsimplex$ to $p_{F-1} \in \compsimplex$ as fixed by a conditional distribution $\pi(x_c|x_c')$, which determines $p_{F-1}$ from $p_1$ by
\begin{equation}
    p_{F-1}(x_c) = \sum_{x_c'\in \mathcal{X}_c} \pi(x_c|x_c') p_1(x_c').
\end{equation}
The conditional distribution $\pi(x_c|x_c')$ can be physically implemented to infinitesimally small error by the time-protocol of the rate matrix $W_{x_c,x_c'}(t)$ \cite[p. 23]{Wolpert2019}\cite{Owen_2019} (assuming $x_c$ [or $x_M$] is extended to include sufficient states, see \cite{Owen_2019}). The notation $p_{F-1} = \pi p_1$ emphasizes that $p_{F-1}$ is purely a function of the input state $p_1$ and the physical manipulations performed by the computation $W_{x_c,x_c'}(t)$, which determines $\pi(x_c|x_c')$.

\subsubsection{Variational MMC and the Island Decomposition}

The requirements to obtain the minimum entropy distribution $q_1$ that returns a unique MMC are specified in \cite{Wolpert_2020}. \cite{Wolpert_2020} points out that uniqueness of optimal distributions can only be verified for `islands' of the conditional distribution defined by the algorithm. 
We can describe an algorithm (possibly stochastic) as implementing a conditional distribution $\pi(x_c | x_c')$ that maps between computational states $x_c,x_c' \in \mathcal{X}_c$. The islands of the algorithm are specified by the following relation for $x_c, x'_c \in \mathcal{X}_c$:
\begin{equation}
    \label{eq:Islands}
    x_c \sim x_c' \Leftrightarrow \exists x_f \in \mathcal{X}_c : \pi(x_f|x_c') > 0, \pi(x_f|x_c) > 0,
\end{equation}
meaning there is a finite probability of $x_c$ and $x_c'$ transitioning to the same state $x_f$. An \textit{island} of $\pi(x_c | x_c')$ is a connected subset of $\mathcal{X}_c$ given by the transitive closure of Eq.~\eqref{eq:Islands}. The set of islands of $\pi$ partition $\mathcal{X}_c$, where the set of islands is denoted $L(\pi)$.

We can consider the distribution over an island $c \in L(\pi)$, given by $p^c(x_c) = \indic{x_c \in c}p(x_c)/p(c)$. If optimized over a the probability simplex specific to the island $c$ is $\boldsymbol{\Delta}_c$, the minimizer $q^c(x)$ will be unique \cite{Wolpert_2020}. The total distribution optimized over $\compsimplex$ can be decomposed in terms of islands and the probability of their individual occupation $q_1(c)$, 
\begin{equation}
    \label{eq:island_dist}
    q_1(x_c) = \sum_{c \in L(\pi)} q_1(c) q_1^c(x_c).
\end{equation}
The factors $q(c)$ do not contribute to the KL divergences in Eq.~\eqref{eq:MMC}, meaning they do not contribute to the MMC and ensuring the MMC is unique for the optimal distribution $q_1$.

For a deterministic algorithm, $\pi$ will be valued 0 or 1 for all inputs. In this case, the islands of the algorithm will be specified by the set of inputs that correspond to a single output state. As we have considered them, both exact linear regression and SGD are deterministic algorithms. In the exact case, the final $\wh_Q$ follows deterministically from the data $\mathcal{D}_Q$, and given that for SGD $\wh_Q$ has a deterministic initialization, the final $\wh_Q$ also follows deterministically from the batches $\{\mathcal{B}_{Q,1},...,\mathcal{B}_{Q,\tau}\}$. Each island of the algorithms corresponds to all possible $\mathcal{D}_Q$ or $\{\mathcal{B}_{Q,1},...,\mathcal{B}_{Q,\tau}\}$ that have the same output $\wh_Q$. For both the exact regression and SGD, the islands of input states are complex but disjoint subsets of the input data, which correspond to specific values of $\Wh$, rendering the island decomposition difficult to consider in this case.

The variational approach breaks the island decomposition by preventing $q_1^c(x_c)$ from being individually optimized, and by preventing a description of the input state as specified by Eq.~\eqref{eq:island_dist}. With a variational $q_{1,v}$ that breaks the island decomposition, we cannot guarantee it to be unique. However, this lack of uniqueness does not prevent MMC$_v$ from providing a lower bound on the true MMC: one can perform a bounded optimization to find $q_{1,v}$, which may or may not be unique, the difference MMC$_v = \Delta S_{tot}(p_{1,v}) - \Delta S_{tot}(q_{1,v})$ will retain the property $0 \leq $ MMC$_v \leq $ MMC for variational distributions $p_{1,v} \in \mathcal{V}$. 

\subsubsection{Illustrative MMC for exact regression and SGD}

\FloatBarrier
\begin{figure}[htbp]
    \centering
    \begin{subfigure}{0.36\textwidth}
        \includegraphics[width=\linewidth]{MMC/MMC_Ex.pdf}
        \caption{}
        \label{fig:MMC_Ex}
    \end{subfigure}
    \begin{subfigure}{0.42\textwidth}
        \includegraphics[width=\linewidth]{MMC/MMC_SGD.pdf}
        \caption{}
        \label{fig:MMC_SGD}
    \end{subfigure}
    \caption{\textit{A lower bound on the mismatch cost for continuously parameterized inputs}. MMC$_v(\sigma_x, \sigma_\xi)$ as a function of $\sigma_x$ and $\sigma_\xi$, with each plot assumes the entropy flow $\Delta S_{env,Ex} = \Delta S_{env, SGD} = C + \alpha(\sigma_x^2 + \sigma_\xi^2 )$, and $w = 1$. A bounded optimization is performed for for $0.75 \leq \sigma_x \leq 5$, $0.5 \leq \sigma_\xi \leq 5$. \ref{fig:MMC_Ex} A sample MMC$_v$ landscape for exact linear regression with the illustrative $\Delta S_{env,Ex}=C + \alpha(\sigma_x^2 + \sigma_\xi^2 )$, and $n = 10$. \ref{fig:MMC_SGD} A sample MMC$_v$ landscape for linear regression via SGD with an illustrative $\Delta S_{env,SGD}=C + \alpha(\sigma_x^2 + \sigma_\xi^2 )$, and $B = 1$, $\tau = 50$.} 
    \label{fig:MMC}
\end{figure}

For exact regression, the variational family will be $\theta = (\sigma_x,\sigma_\xi)$, which only runs from inputs to outputs once, $\Delta S_{tot}$ will be
\begin{equation}
    \Delta S_{tot, Ex}(\sigma_x, \sigma_\xi) = -E^{Ex}_{min}(\sigma_x,\sigma_\xi)/T+\Delta S_{env,Ex}(\sigma_x,\sigma_\xi)
\end{equation}
from which $q_{1,v}(\sigma_x^\star,\sigma_\xi^\star)$, defined by the optimal $\sigma_x^\star$ and $\sigma_\xi^\star$, follows from Eq.~\eqref{eq:mmc_var_opt}. MMC$_v$ for exact regression is given by MMC$_v(\sigma_x,\sigma_\xi) = \Delta S_{tot, Ex}(\sigma_x,\sigma_\xi) - \Delta S_{tot,Ex}(\sigma_x^\star,\sigma_\xi^\star)$. Fixing $\Delta S_{env,Ex} = C+\alpha(\sigma_x^2 + \sigma_\xi^2)$, MMC$_v$ is plotted for a range of distributions in Fig.~\ref{fig:MMC_Ex}.

For the SGD device, each update cycle $k$ takes input $(\mathcal{B}_Q, \hat{W}_{Q,k})$ and produces
output $\hat{W}_{Q,k+1}$, constituting a separate physical process. The MMC should
therefore be evaluated at each step and summed,
\begin{equation}
    \mathrm{MMC}_{v,\mathrm{SGD}}(\sigma_x,\sigma_\xi) = \sum_{k=0}^{\tau-1} \Bigl(\Delta S_{tot, k}(\sigma_x,\sigma_\xi) - \Delta S_{tot,k}(\sigma_x^\star,\sigma_\xi^\star)\Bigr),
\end{equation}
where the per-step total entropy production is
\begin{equation}
    \Delta S_{\mathrm{tot},k}(\sigma_x, \sigma_\xi)
    = 
    - k_B \ln[2]\left(H(\hat{W}_{Q,k}) + B H(X_{fp}, Y_{fp})
      - H(\hat{W}_{Q,k+1})\right) + \Delta S_{env,SGD}.
\end{equation}
To simplify this expression, we can assume that the entropy flow at each step depends only
on the batch distribution, and not on the evolving model parameter distribution,
\begin{equation}
    \Delta S_{env,k}(\theta) = \Delta S_{env,Ex}(\theta)/\tau =  (C + \alpha(\sigma_x^2 + \sigma_\xi^2))/\tau \quad \forall\, k.
\end{equation}
This reduces the per-step sum to a telescoping series as in the preliminaries, giving the total entropy production
\begin{equation}
    \Delta S_{tot,\mathrm{SGD}}(\sigma_x,\sigma_\xi) = -E^{SGD}_{min}(\sigma_x,\sigma_\xi)/T + \Delta S_{env,SGD}(\sigma_x,\sigma_\xi),
\end{equation}
and thus $\mathrm{MMC}_{v,\mathrm{SGD}}(\sigma_x,\sigma_\xi) = \Delta S_{tot,\mathrm{SGD}}(\sigma_x,\sigma_\xi) - \Delta S_{tot,\mathrm{SGD}}(\sigma_x^\star,\sigma_\xi^\star)$.
Fixing $\Delta S_{env}$ beyond its reversible bound cannot be done at an algorithmic level. While we leave evaluation of the true entropy flow $\Delta S_{env}$ to future work, we can demonstrate an example of this approach using an illustrative choice of the entropy flow: $\Delta S_{env}(\sigma_x,\sigma_\xi) = \Delta S_{env,Ex}(\sigma_x,\sigma_\xi) = \Delta S_{env,SGD}(\sigma_x,\sigma_\xi) = C + \alpha(\sigma_x^2 + \sigma_\xi^2)$, as shown in Fig.~\ref{fig:MMC}. 


\pagebreak
\FloatBarrier


==> appendices/prob_dist_z.tex <==
\section{Computing the Probability Distribution of Z}\label{sec:compute_f_z}

\begin{lemma}
    \label{lem:compute_f_z}
    Let $\bX \sim \mathcal{N}(0, \sigx^2 I_n)$ and $\bXi \sim \mathcal{N}(0, \sigxi^2 I_n)$ be independent, with $n \in \mathbb{N}$, and define $Z = \frac{\bX^T\bXi}{\bX^T\bX}$. The probability density function of $Z$ is
\begin{align}
    f_Z(z) = \sqrt{\frac{1}{\pi\paren{\sigx^2}^n\sigxi^2}}\frac{\Gamma\paren{\frac{n+1}{2}}}{\Gamma\paren{\frac{n}{2}}}\paren{\frac{\sigx^2\sigxi^2}{\sigx^2z^2 + \sigxi^2}}^{\frac{n + 1}{2}}
\end{align}
which is the probability density function of a scaled Student's t-distributed random variable with $n$ degrees of freedom and a scale of $\frac{\sigxi}{\sigx\sqrt{n}}$ \cite{JohnsonNormanLloyd1994Cud}. 
\end{lemma}

\begin{proof}[Proof of Lemma~\ref{lem:compute_f_z}]
Recall that $Z = \frac{\xv^T\xiv}{\xtx}$. Using the law of total probability, we have
\begin{align}
    f_{Z}(z) &= \int f_{Z|\xv} (z|\xv)f_\xv(\xv)d\xv.
\end{align}
We see that $f_{Z|\xv} (z|\xv) \sim \gauss{0}{\frac{\sigxi^2}{\xv^T\xv}}$. Let $\xt \sim \gauss{0}{\frac{\sigx^2\sigxi^2}{\sigx^2z^2 + \sigxi^2}I}$. This means,
\begin{align}
    f_{Z}(z) &= \int \frac{\sqrt{\xtx}}{\sqrt{2\pi\sigxi^2}}e^{\frac{-(\xv^T\xv)z^2}{2\sigxi^2}}\paren{\frac{1}{\sqrt{2\pi\sigx^2}}}^ne^{-\frac{\xv^T\xv}{2\sigx^2}} d\xv\\
    &= \frac{1}{\sqrt{2\pi\paren{\sigx^2}^n\sigxi^2}}\paren{\frac{\sigx^2\sigxi^2}{\sigx^2z^2 + \sigxi^2}}^{\frac{n}{2}}\int \sqrt{\xtx}\paren{\frac{1}{\sqrt{2\pi}}}^n \paren{\frac{\paren{\sigx^2}^n\sigxi^2}{\sigx^2z^2 + \sigxi^2}}^{-\frac{n}{2}} e^{-\frac{\xtx}{2}\bracket{\frac{z^2}{\sigxi^2} + \frac{1}{\sigx^2}}}d\xv\\
    &= \frac{\E{\sqrt{\xttxt}}}{\sqrt{2\pi\paren{\sigx^2}^n\sigxi^2}}\paren{\frac{\sigx^2\sigxi^2}{\sigx^2z^2 + \sigxi^2}}^{\frac{n}{2}}.
\end{align}

Let $c \triangleq \frac{\sigx^2\sigxi^2}{\sigx^2z^2 + \sigxi^2}$ and let $\mathbf{g} \sim \mathcal{N}(0, I_n)$. We have $\E{\sqrt{\xttxt}} = \sqrt{c}\,\E{\sqrt{\mathbf{g}^T\mathbf{g}}} = \sqrt{2c}\frac{\Gamma\paren{\frac{n+1}{2}}}{\Gamma\paren{\frac{n}{2}}}$, where the last equality uses $\sqrt{\mathbf{g}^T\mathbf{g}} \sim \chi(n)$ \cite{JohnsonNormanLloyd1994Cud}. Therefore,
\begin{align}
    f_Z(z) &= \sqrt{\frac{1}{\pi\paren{\sigx^2}^n\sigxi^2}}\sqrt{\frac{\sigx^2\sigxi^2}{\sigx^2z^2 + \sigxi^2}}\frac{\Gamma\paren{\frac{n+1}{2}}}{\Gamma\paren{\frac{n}{2}}}\paren{\frac{\sigx^2\sigxi^2}{\sigx^2z^2 + \sigxi^2}}^{\frac{n}{2}}\\
    &= \sqrt{\frac{1}{\pi\paren{\sigx^2}^n\sigxi^2}}\frac{\Gamma\paren{\frac{n+1}{2}}}{\Gamma\paren{\frac{n}{2}}}\paren{\frac{\sigx^2\sigxi^2}{\sigx^2z^2 + \sigxi^2}}^{\frac{n + 1}{2}}\label{eq:f_z_appendix}
\end{align}
This distribution is depicted in Fig.~\ref{fig:z_fit} for varying values of $n$.
\end{proof}


\begin{figure}[htbp]
  \centering
  \begin{subfigure}{0.33\textwidth}
    \centering
    \includegraphics[width=\linewidth]{Exact/slope_fit_distribution_N=3.pdf}
    \caption{$n = 3$}
    \label{fig:z_fit_3}
  \end{subfigure}\hfill
  \begin{subfigure}{0.33\textwidth}
    \centering
    \includegraphics[width=\linewidth]{Exact/slope_fit_distribution_N=10.pdf}
    \caption{$n=10$}
    \label{fig:z_fit_10}
  \end{subfigure}\hfill
  \begin{subfigure}{0.33\textwidth}
    \centering
    \includegraphics[width=\linewidth]{Exact/slope_fit_distribution_N=30.pdf}
    \caption{$n=30$}
    \label{fig:z_fit_30}
  \end{subfigure}
  \caption{\textit{The probability density function} $f_Z(z)$, with $\sigx = \sigxi = 1$. As $n$ increases, the distribution becomes more peaked around $z = 0$. The simulation is of 50000 trials.} 
  \label{fig:z_fit}
\end{figure}

\FloatBarrier
\pagebreak


==> appendices/scaling_laws_app.tex <==
\section{Derivations for Energy-cost Aware Scaling Laws}\label{sec:scaling_laws_app}

\subsubsection{Exact Formula}
Using the generalization error scaling for the exact linear regression formula in Eq.~\eqref{eq:exact_error}, we can solve a continuous relaxation of the optimization problem in Eq.~\eqref{eq:scaling_opt} where $\tilde n \in \R{}$. Let \begin{equation}\label{eq:u_ex}
u_{Ex}(\tilde n) \triangleq \rho_I\frac{\tilde n-2}{(\tilde n-1)\sigxi^2} - \rho_{J}\Delta E_{min}^{Ex}\paren{\tilde n}.
\end{equation}
 The optimization problem now becomes
\begin{align}
    \tilde n^\star &= \arg\max\limits_{\tilde n \geq 3} u_{Ex}(\tilde n) \text{, and } \nonumber\\
    n^\star &= \arg\max_{n\in\{\lfloor \tilde n^\star\rfloor,\lceil \tilde n^\star\rceil\}} u_{Ex}(n)\label{eq:nstar_ex}.
\end{align}
For simplicity, assume $|w| \gg \frac{\sigxi}{\sigx}$. Although the following method could be derived using the exact entropy calculations in Sections~\ref{sec:fpn}~and~\ref{sec:exact}, we will use $\tilde H_s(\Xfp, \Yfp)$ from Eq.~\eqref{eq:approx_joint_ent_SNR} and $\tilde H^w_s(\Wh_{fp}) = h(Z) + (p-1) -\log\bracket{\frac{|w|}{\sqrt{2}}}$ in this section for tractability. $h(Z)$ is computed in Lemma~\ref{lem:diff_ent_Ex}. Let $\psi^\prime(x) \triangleq \frac{d}{dx}\psi(x)$. Taking the derivative of $u$ with respect to $\tilde n$, we have
\begin{align}
    u^\prime_{Ex} (\tilde n) &= \frac{\rho_I}{\sigxi^2}\paren{\frac{1}{\tilde n-1}}^2\nonumber - \rho_J k_BT \ln[2] \paren{2\Ht^0_{s}(p) - \frac{1}{2}\log\bracket{ 1 + \frac{\sigma^2_x w^2}{\sigma_\xi^2}}- \frac{d}{d\tilde n}h(Z)}\label{eq:ddn_profit_ex},
\end{align}
where
\begin{align}
    \frac{d}{d\tilde n}h(Z) &= \log\bracket{e}\paren{\frac{\tilde n+1}{4} }\left(\psi^\prime\left(\frac{\tilde n+1}{2}\right)-\psi^\prime\left(\frac{\tilde n}{2}\right)\right).
\end{align}

It is not guaranteed that Eq.~\eqref{eq:ddn_profit_ex} will have a solution for all settings of parameters. It is recommended to solve the equation numerically using a root finder.\footnote{In our simulations, the profit function appears to be unimodal in $n$ which would justify the rounding procedure given in Eq.~\eqref{eq:nstar_ex}. We leave the proof of this unimodality for future work.} In Fig.~\ref{fig:ddn_profit_ex} we can see where $u^\prime_{Ex} (\tilde n)$ crosses zero for various setting of the price of energy $\rho_J$ and these zero crossings correspond to maximum values of the profit $u_{Ex}(n)$.

\subsubsection{Stochastic Gradient Descent}
\begin{figure}[bthp]
  \centering
  \begin{subfigure}{0.49\textwidth}
    \centering
    \includegraphics[width=\linewidth]{code/scaling/u_sgd_vary_eta.pdf}
    \caption{}
    \label{fig:profit_sgd_eta}
  \end{subfigure}
  \begin{subfigure}{0.49\textwidth}
    \centering
    \includegraphics[width=\linewidth]{code/scaling/u_sgd_vary_B.pdf}
    \caption{}
    \label{fig:profit_sgd_B}
  \end{subfigure}
  \begin{subfigure}{0.49\textwidth}
    \centering
    \hspace*{-0.35cm} 
    \includegraphics[width=\linewidth]{code/scaling/u_prime_sgd_vary_eta.pdf}
    \caption{}
    \label{fig:ddn_profit_sgd_eta}
  \end{subfigure}
  \begin{subfigure}{0.49\textwidth}
    \centering
    \hspace*{-0.35cm} 
    \includegraphics[width=\linewidth]{code/scaling/u_prime_sgd_vary_B.pdf}
    \caption{}
    \label{fig:ddn_profit_sgd_B}
  \end{subfigure}
  \caption{\textit{The effect of the learning rate and batch size on the optimal dataset size for stochastic gradient descent.} (\ref{fig:profit_sgd_eta}) shows $u_{SGD}(n)$ given in Eq.~\eqref{eq:u_sgd} for varying values of the learning rate $\eta$. Notice that smaller learning rates lead to larger optimal dataset sizes. (\ref{fig:ddn_profit_sgd_eta}) shows $u'_{SGD}(n)$ in Eq.~\eqref{eq:ddn_profit_sgd} for the different learning rates. (\ref{fig:profit_sgd_B}) shows $u_{SGD}(n)$ for various values of the batch size $B$. For the profit plots, the gold stars are the maximum values of the profit with respect to each algorithm's feasible set for each value of $\eta$ or $B$. (\ref{fig:ddn_profit_sgd_B}) shows $u'_{SGD}(n)$ for the different batch sizes. The vertical dotted lines show the point where each curve crosses zero. For all figures, $\sigxi^2 =\sigx^2 = 1$, $k_BT = 4\times 10^{-21}$, $w = 2$, $\wh_0 = 1$, $\rho_I = 10$, and $\rho_J = 5\times 10^{16}$. For the plots that vary $\eta$, $B=10$ and for the plots that vary $B$, $\eta = 0.05$.}
  \label{fig:scaling_laws_sgd_eta_B}
\end{figure}
For stochastic gradient descent, we can again take a continuous relaxation of the optimization problem in Eq.~\eqref{eq:scaling_opt}. Let 
\begin{equation}\label{eq:u_sgd}
u_{SGD}(\tilde n) \triangleq \rho_I\paren{\sigx^2\bracket{\frac{\eta\sigxi^2}{2B}\paren{1 -e^{-\frac{2\sigx^2 \eta \tilde n}{B}}} + \paren{\tilde \mu\paren{\frac{\tilde n}{B}} - w}^2} + \sigxi^2}^{-1} - \rho_J \Delta E_{min}^{SGD}\paren{\frac{\tilde n}{B}},
\end{equation} 
to obtain the optimization problem
\begin{align}
    \tilde n^\star &= \arg\max\limits_{\tilde n \geq B} u_{SGD}(\tilde n) \text{, and } \nonumber\\
    n^\star &= \arg\max_{n\in\{B\lfloor \tilde n^\star/B\rfloor,\, B\lceil \tilde n^\star/B\rceil\}} u_{SGD}(n)\label{eq:nstar_sgd},
\end{align}
where the rounding ensures $n^\star \in B\N{}$, since the total number of SGD training samples must satisfy $n = kB$ for integer $k$.
Under the assumptions that the learning rate $\eta$ is small enough that $|\tilde \mu(k)| \gg \sqrt{\frac{\eta\sigxi^2}{2B}}$ throughout the optimization domain, and that $k$ is large enough for the OU approximation Eq.~\eqref{eq:langevin} to track the true SGD dynamics (see Section~\ref{sec:nonstationarysgd}), we can use the approximate entropy $\Ht^{\tilde \mu(k)}_s(\Wh_{fp,k})$ given in Eq.~\eqref{eq:three_approxes}. Taking the derivative of $u_{SGD}$ with respect to $\tilde n$, we have
\begin{align}
    &u^\prime_{SGD} (\tilde n) = -\rho_I\frac{\eta  \sigx^4 e^{-\frac{2 \eta  \tilde n \sigx^2}{B}} \left(\eta  \sigxi ^2-2 B (w-\wh_0)^2\right)}{B^2\paren{\sigx^2\bracket{\frac{\eta\sigxi^2}{2B}\paren{1 -e^{-\frac{2\sigx^2 \eta \tilde n}{B}}} + \paren{\tilde \mu\paren{\frac{\tilde n}{B}} - w}^2} + \sigxi^2}^{2}} \nonumber\\
    &- \rho_J k_BT \ln[2] \Bigg(2\Ht^0_{s}(p) - \frac{1}{2}\log\bracket{ 1 + \frac{\sigma^2_x w^2}{\sigma_\xi^2}}+ \frac{\eta  \sigx^2  \left(w \left(1-e^{-\frac{\eta  \tilde n \sigx^2}{B}}\right)-\wh_0 \right)}{B \ln\bracket{2} \left(1 - e^{-\frac{2 \eta  \tilde n \sigx^2}{B}}\right) \left(w \left(e^{\frac{\eta  \tilde n \sigx^2}{B}}-1\right)+\wh_0\right)}\Bigg).\label{eq:ddn_profit_sgd}
\end{align}

Similar to the exact formula case, in Fig.~\ref{fig:ddn_profit_sgd} we plot $u^\prime_{SGD} (n)$ for various $\rho_J$ and show that its zero crossings correspond to maxima in  $u_{SGD} (n)$ in Fig.~\ref{fig:profit_sgd}. The optimal dataset size decreases as $\rho_J$ increases.




\pagebreak
\FloatBarrier


==> appendices/sgd_fit_quality.tex <==
\section{SGD Fit Quality}

Here we review the fit quality of approximations introduced to obtain analytic expressions for the entropy of model parameters along stochastic gradient descent. Fig.~\ref{fig:assymp_fit} shows the asymptotic fit quality, while Fig.~\ref{fig:non_assymp_fit} shows the nonasymptotic fit quality.

\begin{figure}[htbp]
  \centering
    \centering
    \includegraphics[width=0.3\linewidth]{stationary/assymp_fit (1).pdf}
  \caption{\textit{Fit quality for asymptotic stochastic gradient descent.} Empirical investigation of the validity of the continuous Ornstein-Uhlenbeck process approximation with a simulation of $\hat w$ with $\eta = 0.01$, $\tau = 200$, $\sigma_x^2 = 1$, and $\sigma_\xi^2=1$, for 1000 trials. From top to bottom, the batch sizes are $B = \{1,5,25\}$ while $\tau = 200$, showing the approximation is already effective for these parameters at low $B$. }
  \label{fig:assymp_fit}
\end{figure}

\begin{figure}[htbp]
  \centering
  \begin{subfigure}{0.42\textwidth}
    \centering
    \includegraphics[width=\linewidth]{code/nonstationary/non_assymp_fit.pdf}
    \caption{}
    \label{fig:non_assymp_fit}
  \end{subfigure}
  \begin{subfigure}{0.3\textwidth}
    \centering
    \includegraphics[width=\linewidth]{code/nonstationary/mean_fit.pdf}
    \caption{}
    \label{fig:mean_fit}
  \end{subfigure}
  \caption{\textit{SGD dynamics for zero-intercept simple linear regression.} (\ref{fig:non_assymp_fit}) SGD parameter $\hat w$ distribution at selected iterations, for 5000 separate trials of running SGD. $\sigx^2 = 1$, $\sigxi^2 = 1$, $\eta = 0.01$, $B = 10$. (\ref{fig:mean_fit}) Theoretical mean and standard deviation compared to the empirical mean and standard deviation as step number $k$ increases up to final value $k = \tau = 2000$.}
  \label{fig:sgd_w_2x2}
\end{figure}

\FloatBarrier
\pagebreak


==> defs.tex <==
% organization
\newcommand{\bracket}[1]{\left[ #1 \right]}
\newcommand{\curly}[1]{\left\{ #1 \right\}}
\newcommand{\paren}[1]{\left( #1 \right)}
\newcommand{\abs}[1]{\left| #1 \right|}

% algebra
\newcommand{\R}[1]{\mathbb{R}^{#1}}
\newcommand{\N}[1]{\mathbb{N}^{#1}}
\newcommand{\Z}[1]{\mathbb{Z}^{#1}}
\newcommand{\C}[1]{\mathbb{C}^{#1}}
\newcommand{\K}[1]{\mathbb{K}^{#1}}
\newcommand{\Sym}[1]{\mathbb{S}^{#1}}
\newcommand{\norm}[2]{\left|\left| #1 \right|\right|_{#2}}
\newcommand{\innprod}[2]{\left\langle #1, #2 \right\rangle}

% probability
\newcommand{\Esub}[2]{\mathbb{E}_{#2}\left[ #1 \right]}
\newcommand{\E}[1]{\mathbb{E}\left[ #1 \right]}
\newcommand{\prob}[1]{\mathbb{P}\left( #1 \right)}
\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}} % independence symbol
\newcommand{\indic}[1]{\mathbbm{1}_{\left\{#1\right\}}} %indicator function
\newcommand{\iid}{\stackrel{iid}{\sim}} % iid


% pdfs and pmfs
\newcommand{\gauss}[2]{\mathcal{N}\paren{#1, #2}}
\newcommand{\bern}[1]{\mathrm{Ber}\paren{#1}}
\newcommand{\bin}[2]{\mathrm{Bin}\paren{#1, #2}}
\newcommand{\pois}[1]{\mathrm{Poisson}\paren{#1}}
\newcommand{\unif}[2]{\mathrm{Unif}\paren{#1, #2}}
\newcommand{\geo}[1]{\mathrm{Geometric}\paren{#1}}
\newcommand{\expon}[1]{\mathrm{Exp}\paren{#1}}
\newcommand{\hypgeo}[4]{\mathrm{HypGeo}\paren{#1, #2, #3, #4}}
% info theory
\newcommand{\alphx}{\mathcal{X}}
\newcommand{\alphy}{\mathcal{Y}}
\newcommand{\mutual}[2]{I\paren{#1;#2}}
\newcommand{\condmutual}[3]{I\paren{#1;#2|#3}}
\newcommand{\ent}[1]{H\paren{#1}}
\newcommand{\condent}[2]{H\paren{#1|#2}}
\newcommand{\jointent}[2]{H\paren{#1,#2}}
\newcommand{\relent}[2]{D\paren{#1||#2}}


%calculus
\newcommand{\del}[2]{\frac{\partial #1}{\partial #2}}

%note
\newcommand{\thinkabout}[1]{\textcolor{blue}{\textbf{think about:} #1}}
\newcommand{\fix}[1]{\textcolor{red}{\textbf{fix:} #1}}
\newcommand{\remember}[1]{\textcolor{magenta}{\textbf{remember:} #1}}


% % organization
% \newcommand{\bracket}[1]{\left[ #1 \right]}
% \newcommand{\paren}[1]{\left( #1 \right)}
% \newcommand{\abs}[1]{\left| #1 \right|}

% % algebra
% \newcommand{\R}[1]{\mathbb{R}^{#1}}
% \newcommand{\N}[1]{\mathbb{N}^{#1}}
% \newcommand{\Z}[1]{\mathbb{Z}^{#1}}
% \newcommand{\C}[1]{\mathbb{C}^{#1}}
% \newcommand{\K}[1]{\mathbb{K}^{#1}}
% \newcommand{\Sym}[1]{\mathbb{S}^{#1}}
% \newcommand{\norm}[2]{\left|\left| #1 \right|\right|_{#2}}
% \newcommand{\innprod}[2]{\left\langle #1, #2 \right\rangle}

% % probability
% \newcommand{\Esub}[2]{\mathbb{E}_{#2}\left[ #1 \right]}
% \newcommand{\E}[1]{\mathbb{E}\left[ #1 \right]}
% \newcommand{\prob}[1]{\mathbb{P}\left( #1 \right)}
% \newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
% \def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}} % independence symbol
% \newcommand{\indic}[1]{\mathbbm{1}_{\left\{#1\right\}}} %indicator function
% % pdfs and pmfs
% \newcommand{\gauss}[2]{\mathcal{N}\paren{#1, #2}}
% \newcommand{\bern}[1]{\mathrm{Ber}\paren{#1}}
% \newcommand{\bin}[2]{\mathrm{Bin}\paren{#1, #2}}
% \newcommand{\pois}[1]{\mathrm{Poisson}\paren{#1}}
% \newcommand{\unif}[2]{\mathrm{Unif}\paren{#1, #2}}
% \newcommand{\geo}[1]{\mathrm{Geometric}\paren{#1}}
% \newcommand{\expon}[1]{\mathrm{Exp}\paren{#1}}
% \newcommand{\hypgeo}[4]{\mathrm{HypGeo}\paren{#1, #2, #3, #4}}
% % info theory
% \newcommand{\alphx}{\mathcal{X}}
% \newcommand{\alphy}{\mathcal{Y}}
% \newcommand{\mutual}[2]{I\paren{#1;#2}}
% \newcommand{\condmutual}[3]{I\paren{#1;#2|#3}}
% \newcommand{\ent}[1]{H\paren{#1}}
% \newcommand{\condent}[2]{H\paren{#1|#2}}
% \newcommand{\jointent}[2]{H\paren{#1,#2}}
% \newcommand{\relent}[2]{D\paren{#1||#2}}


% %calculus
% \newcommand{\del}[2]{\frac{\partial #1}{\partial #2}}


==> sections/exact_lr.tex <==
\section{Landauer Cost of Exact Linear Regression}\label{sec:exact}

We now will compute the Landauer cost of exact simple linear regression, assuming all continuous variables are implemented on single-precision floating-point numbers, with $E = 8$, $p=24$. The optimal fit line $\wh$ is determined by exact linear regression formula Eq.~\eqref{eq:exact_formula}, and is computed from the entire data set. With each of $n$ data points being independent and identically distributed, if we assume the distribution is sufficiently slow varying for the $p=24$ case (as supported by Fig.~\ref{fig:fp_joint_exact_approx_p_E_snr_100}, where the $p=4$ case will have even finer bins), and that the overflow and underflow probabilities are low, the entropy of the input data can be approximated using Eq.~\eqref{eq:approx_joint_ent_SNR}: 
\begin{equation}\label{eq:input_ent_ex}
    H(\mathcal{D}_{fp}) = nH(\Xfp, \Yfp) \approx n \Ht_s(X_{fp}, Y_{fp}).
\end{equation}

For the output data, $\Wh = \frac{\bX^T\bY}{\bX^T\bX}$ is the predicted slope using the exact formula for linear regression. The differential entropy of the predicted slope is
\begin{align}
h(\Wh) &= h\paren{\frac{\bX^T\bY}{\bX^T\bX}} = h\paren{\frac{\bX^T(w\bX + \bXi)}{\bX^T\bX}} = h\paren{w + \frac{\bX^T\bXi}{\bX^T\bX}} = h\paren{\frac{\bX^T\bXi}{\bX^T\bX}},
\end{align}
since $w$ is a constant. From Lemma~\ref{lem:compute_f_z}, if $Z = \frac{\bX^T\bXi}{\bX^T\bX}$, the probability density function of $Z$ is
\begin{align}
    f_Z(z) = \sqrt{\frac{1}{\pi\paren{\sigx^2}^n\sigxi^2}}\frac{\Gamma\paren{\frac{n+1}{2}}}{\Gamma\paren{\frac{n}{2}}}\paren{\frac{\sigx^2\sigxi^2}{\sigx^2z^2 + \sigxi^2}}^{\frac{n + 1}{2}}\label{eq:exact_final_dist}
\end{align}
which is the probability density function of a scaled Student's t-distributed random variable with $n$ degrees of freedom and a scale of $\frac{\sigxi}{\sigx\sqrt{n}}$ \cite{JohnsonNormanLloyd1994Cud}. 
See Appendix~\ref{sec:compute_f_z} for a proof. Fig.~\ref{fig:z_fit} in App.~\ref{sec:compute_f_z} shows $f_Z(z)$ for different $n$ along with a histogram of the empirical $z$ over 50000 trials. With $\E{Z} = 0$ for $n > 1$ and $\mathrm{Var}(Z) = \frac{\sigxi^2}{\sigx^2}\paren{\frac{1}{n-2}}$ for $n > 2$ \cite{JohnsonNormanLloyd1994Cud}, as $n$ increases the distribution narrows and peaks around zero.
The discrete entropy of $\Wh_{fp}$ is given by Theorem~\ref{thm:quantized_ent} where the cumulative distribution of the scaled and translated Student's t \cite{JohnsonNormanLloyd1994Cud}
\begin{equation}\label{eq:wh_cdf}
F_{\Wh}(\wh) = \frac{1}{2} + \frac{(\wh-w) \sigma_x \Gamma \left(\frac{n+1}{2}\right)}{\sqrt{\pi } \sigma_\xi \Gamma \left(\frac{n}{2}\right)} \, _2F_1\left(\frac{1}{2},\frac{n+1}{2};\frac{3}{2};-\frac{(\wh-w)^2 \sigma_x^2}{\sigma_\xi^2}\right)
\end{equation}
is used and the representable values of the floating-point representation given in Corollary~\ref{cor:gauss_fp_ent}. 















In this case, for $n > 2$ and $|w| \gg \frac{\sigxi}{\sigx\sqrt{n-2}}$, $H(\Wh_{fp}) \approx \Ht_s^w(\Wh_{fp})$ is applied, where the resulting entropy is shown in Fig.~\ref{fig:H_fp_wh} as $n$ increases for various values of the ground truth $w$. The quality of the approximation in this case is justified by its offset from 0, and for high $n$ that the distribution approximates a delta function (App.~\ref{app:FPN_app3}), as well as by the fine bin size provided by $p=24$. Fig.~\ref{fig:H_fp_wh_exact} in App.~\ref{sec:compute_h_z} shows the quality of the approximation $\Ht^\mu_s(\Wh_{fp})$ for $p=4$ floating point numbers when the exact entropy is computable, that the approximation still applies fairly well even for low $n$, which should only improve as $p$ increases. Taking the difference between the input and output entropies, we find the Landauer cost of exact linear regression as specified by Eq.~\eqref{eq:exact_landauer}, and applying Eqs.~\eqref{eq:first_two_approx} and~\eqref{eq:three_approxes}:
\begin{equation}
    \Delta E_{min}^{Ex} \approx k_BT\ln[2]\paren{n\Ht_s(X_{fp},Y_{fp}) - \Ht^w_{s}(\Wh_{fp})}, \label{eq:landauer_exact_lr}
\end{equation}




This result and the entropies that contribute to it are shown in Fig.~\ref{fig:ex_landauer}. Note from Eqns.~\eqref{eq:three_approxes}, \eqref{eq:single_mean_0}, and~\eqref{eq:approx_joint_ent_SNR} that the precision $p$ of the floating-point representation is a significant contributor to the entropy. In Fig.~\ref{fig:Ex_dH} we plot this contribution alone as well, given by $\Delta E^{Ex}_{p} = k_BT \ln[2](2n - 1)p$.





\begin{figure}[htbp]
  \centering
  \begin{subfigure}{0.4\textwidth}
    \centering
    \includegraphics[width=\linewidth]{code/quantized_entropy_midpoint/exact_lr/bigmantissa_approx_H_wh_fp_vs_n.pdf}
    \caption{}
    \label{fig:H_fp_wh}
  \end{subfigure}
  \begin{subfigure}{0.4\textwidth}
    \centering
    \includegraphics[width=\linewidth]{code/quantized_entropy_midpoint/exact_lr/bigmantissa_approx_landauer_cost_per_n_vs_n.pdf}
    \caption{}
    \label{fig:Ex_dH}
  \end{subfigure}\hfill
  \caption{\textit{The Landauer cost for exact zero-intercept simple linear regression.} Input and output states are floating-point numbers with $p = 24$ and $E=8$. The candidate values of the $SNR = w^2\sigx^2/\sigxi^2$ are $0.062$, $0.25$, $1$, $4$, and $25$. (\ref{fig:H_fp_wh}) The output model approximate entropy $\Ht_s^w(\Wh_{fp})$, and its dependence on the number of data samples $n$. (\ref{fig:Ex_dH}) The approximate entropy difference rate between the input data and the output model for various values of $n$. The contribution of the precision of the data $p$ plotted here is $\Delta E^{Ex}_{p}/( k_BT \ln[2]n) =(2n - 1)p/n$ as the gray dots. The joint entropy of the input data is plotted as the dashed horizontal lines for each $SNR$ value.} 
  \label{fig:ex_landauer}
\end{figure}

Fig.~\ref{fig:ex_landauer} shows us the main contributors to the entropy of the output state, and to the overall lower bound on thermodynamic cost. As $n$ increases, the entropy of the output model $\hat w$ decreases (after $n>2$ Fig.~\ref{fig:H_fp_wh}), while the entropy of the input increases with more data. This confirms that thermodynamic costs are higher with more data, and that for large $n$, the entropy of the input data dominates that of the output model. The Landauer cost is nearly linear in $n$ beyond small values with the slope approaching the joint entropy of the input data, as shown in Fig.~\ref{fig:Ex_dH} where Eq.~\eqref{eq:landauer_exact_lr} is scaled by $1/n$ to demonstrate the contribution of the output entropy at low $n$. 

The contribution of the precision $p$ to the Landauer cost is
\begin{equation}
    \label{eq:precision_contribution_Ex}
    \Delta E^{Ex}_{p} \triangleq k_BT \ln[2]\,(2n - 1)p.
\end{equation}
For high $n$, at $p=24$ this is the main contributor to the cost, by approximately $90\%$.\footnote{This effect is even more extreme when analyzing the Landauer cost of averaging and summing normally distributed variables in Appendix~\ref{sec:avg_sum}. In this simpler setting, the only contributors to the Landauer cost are the size of the dataset $n$ and the precision of the data $p$.} Beyond this, the higher the signal-to-noise ratio, the lower the thermodynamic cost.\footnote{For arbitrarily high signal-to-noise ratio, the approximation will eventually break down due to quantization noise as seen in Fig.~\ref{fig:fp_joint_exact_approx_p_E_snr_100}. However, for $p=24$ and the highest SNR considered here being 25, we are well within the bounds of the approximation's applicability.}

     





==> sections/fpn_entropy.tex <==
\section{The Structure of a Floating-point Number}
\label{sec:structure}
% In digital hardware, numerical values are stored as bit strings in finite registers, coming in many forms. Two examples are integers, uniformly spaced values with a range specified by the number of bits, and floating-point numbers, which uses a finite register of binary bits to represent a real value $x$ in binary scientific notation. 
% Here, we focus on floating-point numbers, due to their ubiquitous role in representing continuous variables, and because floating point numbers play a central role in modern deep learning algorithms and hardware \cite{nvidia_nvidia_2025, advanced_micro_devices_inc_amd_2025}. 
% As deep neural network training and inference loads attempt to saturate the computational resources of specialized hardware, there has been renewed interest in developing novel floating-point formats that find the right tradeoffs between precision, dynamic range, memory, computational speed and numerical stability \cite{kuzmin_fp8_2022}.
% Some examples are microscaling (MX) formats \cite{rouhani_microscaling_2023, darvish_rouhani_shared_2023, su_characterization_2025} where $k$ numbers are represented with a single shared exponent that encodes the scale of the block, and $k$ scalar elements that are encoded using 8 bit or less floating point or integer formats.\footnote{An example is MXFP8 where a block has $32$ elements with a shared 8-bit exponent and each scalar element is encoded with FP8 using four exponent bits and three significand bits.} 
\begin{table*}[t]
    \centering
    \renewcommand{\arraystretch}{1.5}
    \begin{tabular}{ccc}
    \hline
    \hline
    Distribution & 
    % Probability Density Function & 
    Approximate entropy: $\tilde H_s(X_{fp}) = p - \frac{1}{2} + h(X) - \mathbb{E}_{f_X}(\log|X|)$ \\
    \hline
    \hline
    
    \hline
    $X \sim \mathcal{N}(0,\sigma^2)$ & 
    % $f_X(x) = \frac{\exp\left(-\frac{x^2}{2\sigma^2}\right)}{\sqrt{2\pi\sigma^2}}, x\in \mathbb{R}$ & 
    $p + \frac{1}{2} \log[2 \pi e] + \frac{\gamma_e}{2\ln[2]}$ \\
    
    $X \sim$ Uniform(-a,a) & 
    % $f_X(x) = \frac{1}{2b}, \ -b \leq x \leq b$ & 
    $ p + \frac{1}{2} +\log(e) $ \\
    
    $X \sim $ Gamma($\alpha,\theta$) & 
    % $f_X(x) = \frac{x^{\alpha-1}e^{-x/\theta}}{\Gamma(\alpha)\theta^\alpha}, \ x>0$ & 
    $ p - \frac{1}{2} + \alpha \log(e)(1 - \psi(\alpha) ) + \log(\Gamma(\alpha))$ \\
    
    $X \sim \chi^2(k)$ & 
    % $f_X(x) = \frac{1}{2^{k/2}\Gamma\left(\frac{k}{2}\right)}x^{\frac{k}{2}-1}e^{-x/2}, \ x>0$ & 
    $p - \frac{1}{2} + \frac{k}{2} \log(e) \bigg (1-\psi \bigg(\frac{k}{2} \bigg) \bigg) + \log \bigg (\Gamma \bigg (\frac{k}{2} \bigg ) \bigg)$  \\
    
    $X \sim$ Laplace(0,b) & 
    % $f_X(x) = \frac{1}{2b}\exp\left(-\frac{|x|}{b}\right), \ x\in \mathbb{R}$ & 
    $p+\frac{1}{2}+ \frac{1+\gamma_e}{\ln2}$ \\
    
    $X \sim$ Logistic(0,s) & 
    % $f_X(x) = \frac{\exp\left(-\frac{x}{s}\right)}{s\left(1+\exp\left(-\frac{x}{s}\right)\right)^2}, \ x\in \mathbb{R}$ & 
    $p-\frac{1}{2}+ \frac{2+\gamma_e - \ln(\pi/2)}{\ln2}$ \\
    
    $X \sim$ Weibull($\lambda,k$) & 
    % $f_X(x) = \frac{k}{\lambda}\left(\frac{x}{\lambda}\right)^{k-1}\exp\left[-\left(\frac{x}{\lambda}\right)^k\right], \ x\geq 0$ & 
    $p-\frac{1}{2}+ \frac{1+\gamma_e}{\ln2} - \log(k)$\\
    
    $X \sim$ Lognormal($\mu, \sigma^2$) & 
    % $f_X(x) = \frac{1}{x\sigma\sqrt{2\pi}}\exp\left[-\frac{(\ln x-\mu)^2}{2\sigma^2}\right], \ x>0$ & 
    $p-\frac{1}{2}+ \log(\sigma \sqrt{2 \pi e})$\\
    
    $X\sim$ Pareto($x_m,\alpha$) & 
    % $f_X(x) = \frac{\alpha x_m^\alpha}{x^{\alpha+1}}, \ x\geq x_m$ & 
    $p-\frac{1}{2}+ \log ( \frac{e}{\alpha} )$\\
    
    $X \sim $ Beta($\alpha,\beta$) & 
    % $f_X(x) = \frac{x^{\alpha-1}(1-x)^{\beta-1}}{B(\alpha,\beta)}, \ 0<x<1$ & 
    $p-\frac{1}{2}+\log B(\alpha,\beta)+\frac{(\alpha+\beta-1)\psi(\alpha+\beta)-\alpha\psi(\alpha)-(\beta-1)\psi(\beta)}{\ln 2}$\\
    
    $X \sim t_{\nu}(0,s)$ & 
    % $f_X(x) = \frac{\Gamma\left(\frac{\nu+1}{2}\right)}{s\sqrt{\nu\pi}\Gamma\left(\frac{\nu}{2}\right)}\left(1+\frac{x^2}{\nu s^2}\right)^{-\frac{\nu+1}{2}}, \ x\in \mathbb{R}$ & 
    $p-\frac{1}{2}
        +\log B\left(\frac{\nu}{2},\frac{1}{2}\right)+
        \frac{\frac{\nu+1}{2}\psi\left(\frac{\nu+1}{2}\right)
        -
        \frac{\nu}{2}\psi\left(\frac{\nu}{2}\right)
        -
        \frac{1}{2}\psi\left(\frac{1}{2}\right)
        }{\ln 2}$ \\
        
    $d$-dimensional multivariate Gaussian & 
    % $(X_1, \dots, X_d) = \Xv \sim \gauss{0}{\Sigma}$ & 
    $d\paren{p+\frac{1}{2}\log\paren{2\pi e} + \frac{\gamma_e}{2\ln[2]}}
        \quad + \frac{1}{2} \log\paren{\frac{\prod\limits_{i=1}^{d}\lambda_i(\Sigma)}{\prod\limits_{i=1}^{d}\Sigma_{ii}}}$\\
    \hline
    \end{tabular}
    \caption{\textit{Closed-form approximations for the discrete entropy of common distributions, quantized on floating-point numbers.} Here we show closed-form expressions approximating the discrete entropy of common distributions when represented on floating-point numbers. $p$ is the precision, $\gamma_e$ is the Euler-Mascheroni constant, $\Gamma(\cdot)$ is the gamma function, $\psi(\cdot)$ is the digamma function, and $B(\cdot, \cdot)$ is the beta function. For the multivariate Gaussian case, we assume scalar quantization in which each component of the random vector is individually quantized on distinct floating-point numbers. Note that for all distributions shown, the scale parameter cancels.}
    \label{tab:closed_form}
\end{table*}
In this paper, we will use a simple normalized floating-point format with midpoint rounding that does not use subnormal numbers (as defined in \cite{muller2010handbookfpn}) and where zero is not in the representable set.

Let $p \in \N{}$, $E \in \N{} \cup \{0\}$, and $\alpha \in \R{}$. The following map is defined on $\R{}\setminus\{0\}$; since all distributions used in this paper are absolutely continuous, the event that the value zero is realized is probability-zero. Define \begin{equation}
    \mathrm{round}_{p}(\alpha) \triangleq \paren{\argmin\limits_{i \in \{0, \dots, 2^{p-1}\}}\abs{\alpha - i2^{-(p-1)}}}2^{-(p-1)},
\end{equation} where ties in the $\argmin$ function are broken towards the higher index $i$. Assuming rounding to the nearest representable value, the value stored on a floating-point number can be written as
\begin{equation}
    x_{fp}(x) \triangleq (-1)^{s_{fp}(x)} \times 2^{e_{fp}(x)} \times \paren{1 + m_{fp}(x)},
\end{equation}
where \begin{equation}
\label{eq:sem_fp}
    \begin{aligned}
        s_{fp}(x) &\triangleq \indic{x < 0},\\
        \tilde e_{fp}(x) &\triangleq -\paren{2^{E-1} - 1}\indic{\log|x| < -\paren{2^{E-1} - 1}}\\
        &+ \sum\limits_{i=0}^{2^E - 1}\bracket{i - \paren{2^{E-1} - 1}}\indic{i - \paren{2^{E-1} - 1} \leq \log|x| < i+1 - \paren{2^{E-1} - 1}} + 2^{E-1}\indic{\log|x| \geq 2^{E-1} + 1}\\
          m_{fp}(x) &\triangleq \mathrm{round}_{p}\paren{|x|2^{-\tilde e_{fp}(x)} - 1}\indic{\log|x| < 2^{E-1}+1}\indic{\mathrm{round}_{p}\paren{|x|2^{-\tilde e_{fp}(x)} - 1
     } \neq 1} \\
          &+ \paren{1 - 2^{-(p-1)} }\paren{\indic{\log|x| \geq 2^{E-1}+1} + \indic{2^{E-1} \leq \log|x| < 2^{E-1}+1}\indic{\mathrm{round}_{p}\paren{|x|2^{-\tilde e_{fp}(x)}
     - 1} = 1}}\\e_{fp}(x) &\triangleq \min\paren{2^{E - 1}, \tilde e_{fp}(x) + \indic{\mathrm{round}_{p}\paren{|x|2^{-\tilde e_{fp}(x)} - 1} = 1}}.
       \end{aligned}\footnote{$\tilde e_{fp}(x)$ must be introduced to handle cases where mantissa value rounds up to the next exponent level. This occurs when $\mathrm{round}
      _{p}\paren{|x|2^{-\tilde e_{fp}(x)} - 1} = 1$.}
   \end{equation}
The quantities in Eq.~\eqref{eq:sem_fp} are decoded numerical values: $s_{fp}(x)$ is a single sign bit, $e_{fp}(x)$ is the binary exponent for $E \geq 1$ (for $E=0$, the format has a single exponent level with implicit exponent value $1/2$), and $m_{fp}$ is the significand (or mantissa) which encodes the binary significant digits of $x$ in the form $1.m_{fp}(x)$; in the physical registers these are encoded as binary integers using $1$, $E$, and $(p-1)$ bits respectively \cite{muller2010handbookfpn, Goldberg1991_FPN_Intro}. Since each stored field is a finite set of non-negative integers constrained by the number of bits in the register, this structure can only represent a finite set $U_{fp}$ of representable numbers along the real number line. For example, the standard single-precision IEEE-754 format uses one bit for $s_{fp}$, 23 bits for $m_{fp}$, and eight bits for $e_{fp}$. Note that the format defined by Eq.~\eqref{eq:sem_fp} is an idealized normalized floating-point format: it does not include zero, subnormal numbers, infinities, or NaNs, and its exponent range ($e_{\min} = -(2^{E-1}-1)$, $e_{\max} = 2^{E-1}$) differs slightly from the IEEE-754 standard. 
The structure of a floating-point number is illustrated in Fig.~\ref{fig:fp_diag}. See \cite{muller2010handbookfpn, Goldberg1991_FPN_Intro} for further details on the floating-point representation.

The purpose of a floating-point number is to store a real number in a discrete state. Thus, for a continuous random variable $X$ loaded onto a floating-point number, our goal will be to find the discrete entropy of its resulting floating-point representation $H(X_{fp})$, where $X_{fp}$ represents the discrete random variable resulting from the floating-point quantization of $X$.  

\section{A Closed-form Approximation for the Entropy of Floating-point Numbers}\label{sec:illustrative_approx}

We can gain significant insight into the entropy of floating-point numbers, as well as a large com analytic expressions for the floating point entropy: relating the discrete entropy of the quantized variable to the differential entropy of the continuous variable, smoothing and extending the bin size function.

These approximations can be compared to direct computation the entropy of a random variable that is clipped and midpoint quantized to representable values. In this case, the probability of each discrete state can be evaluated through numerical integration of the distribution over the quantization range of each representable value.

\textcolor{red}{Add discussion of how to compute exact entropy}

Then, Corollary~\ref{cor:gauss_fp_ent} finds the representable values of the floating-point representation given in Eq.~\eqref{eq:sem_fp}, which can be directly applied to Theorem~\ref{thm:quantized_ent} to directly compute the entropy of $\Xfp$. Due to their length, these exact expressions can be found in App.~\ref{app:exact_entropy_float}. Nevertheless, their numerical evaluations can be seen in Figures~\ref{fig:fp_exact_approx} and~\ref{fig:full_fp_exact_approx_p_E} which support the analysis of following approximations.


\subsubsection*{Approximation 1 -- Relating discrete and differential entropy}

The first approximation relates the differential entropy of a continuous random variable to the discrete entropy of its counterpart discrete representation. This has been studied by \cite{CoverThomas, renyi_dimension_1959, jaynes_information_1962, Jaynes1968-limiting, linder_asymptotic_1994, gish_asymptotically_1968, kostina_data_2017}, focusing on when the quantization uses uniform bins of size $\Delta \in \R{}$. This results in the well known relationship $H(X_Q) \approx h(X) - \log \Delta$, where $h(X) = - \int f_X(x) \log f_X(x) dx$ is the differential entropy. 

However, the formalism in \cite{kostina_data_2017} can be extended to non-uniform bins, and applied to the case of floating-point numbers. In App.~\ref{app:FPN_app1}, the relationship between the differential and discrete entropy is derived for the non-uniform quantization of a $d$-dimensional distribution on $d$ independent registers. For simplicity, here we can focus on the case of a univariate distribution where $d=1$. Assuming bounded support on the region of $\R{}$ bounded by the granular region (see \cite{GrayNeuhoff1998Quantization}) $\mathbb{U} \triangleq [-2^{e_{max} + 1} + 2^{e_{max} - p}, \,\, 2^{e_{max} + 1} - 2^{e_{max} - p}]$, where $e_{max} = 2^{E-1}$. Approximation 1 is $H(X_Q) \approx \tilde H(X_Q)$, where
\begin{equation}
    \label{eq:diff_approx}
    \tilde H(X_Q) \triangleq -\int_\mathbb{U} f_X(x) \log [f_X(x) \Delta(x)] dx = h(X) - \Esub{\log[\Delta(x)]}{\mathbb{U}},
\end{equation}
and $\Esub{\cdot}{\mathbb{U}}$ denotes expectation over the granular region $\mathbb{U}$. As discussed in App.~\ref{app:FPN_app1} and \cite{kostina_data_2017}, approximation 1 is valid if $f_X(x)$ varies slowly over each bin, meaning $f_{X}(x)$ is well approximated by a piecewise distribution which is uniform over each bin (see Fig.~\ref{fig:fp_joint_exact_approx_p_E_snr_100}). 

This expression can be understood through E.T. Jaynes' work on the ``limiting density of discrete points" \cite{Jaynes1968-limiting}. Jaynes emphasized that differential entropy by itself is not an absolute quantity\footnote{While the primary motivation for introducing a discrete representation is the reality that modern computers use discrete representation, the known pathologies of differential entropy also make its application to a cyclic device difficult. Differential entropy is coordinate dependent (as noted by Jaynes \cite{Jaynes1968-limiting}), and it can diverge to $h(X) \rightarrow - \infty$ for sufficiently narrow distributions. Since the standard accounting convention assumes registers are re-initialized to specific, i.e. infinitely narrow states during the computation, use of the differential entropy would not be possible.}, depending implicitly on a reference measure that specifies how the continuous space is discretized. The position dependent bin density provides us with this underlying measure, by specifying the density of states along the number line as $1/\Delta(x)$ \cite{Jaynes1968-limiting}.





\subsubsection*{Approximation 2 -- Smoothing the bin size function and extending its domain}

For floating-point numbers, the spacing between adjacent representable values is constant inside each exponent block. When the value to be quantized $x$ is within the range $[2^{e_{fp}(x)}, 2^{e_{fp}(x)+1})$, a floating-point number can represent $2^{(p-1)}$ equally spaced values. Thus for $2^{e_{fp}(x)} \leq x < 2^{e_{fp}(x)+1}$, meaning that $x$ is in a bin in the interior of an exponent block, the bin size is, 
\begin{equation}
    \label{eq:true_bins}
    \Delta(x) = \frac{2^{e_{fp}(x)+1} - 2^{e_{fp}(x)}}{2^{p-1}}= 2^{e_{fp}(x) - (p-1)} \text{ if }x \in \mathbb{U}.
\end{equation}
In the main text, only the bin size when $x$ is in an interior bin is given for readability; the true midpoint bin-size function $\Delta(x)$ from App.~\ref{app:FPN_app1} takes on different values when $x$ is in the two outer clipping bins, the exponent-boundary bins and the two bins adjacent to zero. These special bins are treated explicitly in App.~\ref{app:FPN_app2}.

Our second approximation will alter the bin size. First we can smooth the steps by introducing a best-fit linear approximation as shown as the dashed red line in Fig.~\ref{fig:fp_diag}, which uses $e_{s}(x) \triangleq \log[|x|/\sqrt{2}]$. This gives us
\begin{equation}
    \label{eq:step_approx}
    \Delta_s(x) \triangleq \frac{1}{\sqrt{2}}|x| \cdot 2^{1-p} \approx \Delta(x).
\end{equation}
By Theorem~\ref{thm:steps}, the error caused by introducing this smooth approximation is bounded by $d/2$ plus the small contribution from the bins adjacent to zero; for most distributions it will be much smaller due to cancellation in the overestimation and underestimation.

Unlike $\Delta(x)$, it is simple to define $\Delta_s(x)$ for any $x \in \mathbb{R}$. With this, and by assuming the probability of overflow and underflow values is small, $\int_{\mathbb{R} \setminus \mathbb{U}} f_X(x) dx \approx 0$, we extend the domain of integration from $\mathbb{U}$ to $\mathbb{R}$. Since $\Delta_s(x)$ grows only linearly in $|x|$, the omitted tail integral $\int_{\mathbb{R}\setminus\mathbb{U}} f_X(x)|\log[f_X(x)\Delta_s(x)]|\,dx$ is near zero for all distributions used in this paper (Gaussian tails decay exponentially and Student's $t$ tails decay as a power law, both of which dominate the linear growth of $\Delta_s$) when the granular region $\mathbb{U}$ is sufficiently large. Approximation 2 states that $\Ht_s(x) \approx \tilde H(x)$ :

\begin{equation}
    \label{eq:first_two_approx}
    \Ht_s(X_{fp}) \triangleq h(X) + (p-1)- \int^\infty_{-\infty} f_X(x) \log\bracket{\frac{|x|}{\sqrt{2}}} dx,
\end{equation}
where $h(X) = -\int^\infty_{-\infty} f_X(x) \log f_X(x) dx$. Approximation 2 applies when $f_X(x)$ has low overflow or underflow probability. Beyond this, the bin-size smoothing error is bounded by $d/2$ plus the small contribution from the bins adjacent to zero (Theorem~\ref{thm:steps}); the domain extension from $\mathbb{U}$ to $\mathbb{R}$ is a separate approximation controlled by the probability mass outside $\mathbb{U}$. Simple and predictive analytic expressions can be obtained using just Eq.~\eqref{eq:first_two_approx} when continuous random variables are Gaussian and centered on 0, as discussed in Section~\ref{sec:gaussians}. 

% \subsubsection*{Approximation 3 -- Evaluating $\mathbb{E}[\log[|x|/\sqrt{2}]]$}

% We can also consider an approximation which can assist with distributions that are not centered at 0. Here we can assume the distribution is offset by a shift, $\mu$. In this case, $\Ht_s(X_{fp})$ will depend on a convolution of $\log[|x|/\sqrt{2}]$ with the probability distribution $f_X(x - \mu)$, 
% \begin{equation}
%     \label{eq:G_int_non_gauss}
%     G_{f_X}(\mu) \triangleq \int^{\infty}_{-\infty} f_X(x-\mu) \log[|x|/\sqrt{2}] dx.
% \end{equation}
% For a smooth distribution which decays rapidly around its mean $\mu$, the resulting integral will approximate a smoothed $\log\bracket{|x|/\sqrt{2}}$ function, as shown for a Gaussian distribution in Fig.~\ref{fig:fp_off_zero}. Approximation 3 states that $\tilde H_s(X_{fp}) \approx \tilde H_s^\mu(X_{fp})$, with
% \begin{equation}
%     \label{eq:three_approxes}
%     \Ht^\mu_s(\Xfp) \triangleq h(X) + (p-1) - \log\bracket{|\mu| / \sqrt{2}}.
% \end{equation}
% This approximation replaces the integral term $G_{f_X}(\mu)$ from Eq.~\eqref{eq:G_int_non_gauss} with $\log[|\mu|/\sqrt{2}]$, and applies for $\mu \neq 0$ when $X \sim \mathcal{N}(\mu, \sigma^2)$ with $|\mu| \gg \sigma$, as well as non-Gaussian distributions which approximate a delta function as a parameter $\epsilon$ defining the distribution's width is decreased toward zero ($\epsilon \to 0$), making the distribution increasingly concentrated around $\mu \neq 0$, as shown in App.~\ref{app:FPN_app3}. The full approximation $H(X_{fp}) \approx \Ht^\mu_s(X_{fp})$ additionally requires that Approximation~1 remains valid, which can fail when the distribution becomes narrower than the quantization bin size. 
% Fig.~\ref{fig:fp_exact_approx_mu} shows this approximation along with the true value of $H(\Xfp)$ as $\mu$ varies.


















% \subsection{Approximating the entropy of a floating-point quantized univariate and bivariate Gaussian}

% \label{sec:gaussians}

% \subsubsection{Univariate Gaussian}
% Applying Eq.~\eqref{eq:first_two_approx}, one can obtain an analytic expression for the approximate discrete entropy of a zero-mean normally distributed continuous random variable $X \sim \mathcal{N}(0, \sigma^2)$ as represented on a floating-point number. By Theorem~\ref{thm:single_gaussian}, $\Ht_s(X_{fp}) = \tilde H^0_s(p)$, where
% \begin{equation}
%     \label{eq:single_mean_0}
%     \Ht^0_{s}(p) \triangleq p + \frac{1}{2} \log[2 \pi e] + \frac{\gamma_e}{2\ln[2]} \approx p + 2.46 \text{ bits}.
% \end{equation}
% $p$ is the precision, and $\gamma_e \approx 0.5772$ is the Euler--Mascheroni constant.

\begin{figure}[htbp]
  \centering
  \begin{subfigure}{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{diagrams/combined_float_diag_bin_size.pdf}
    \caption{}
    \label{fig:fp_diag}
  \end{subfigure}
  \begin{subfigure}{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{code/quantized_entropy_midpoint/sigma_p_E/entropy_sigma_midpoint_p3.pdf}
    \caption{}
    \label{fig:fp_exact_approx_sigma}
  \end{subfigure}
  \begin{subfigure}{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{code/quantized_entropy_midpoint/mu_p_E/entropy_mu_midpoint_sigma_1.0_p_7_E_7.pdf}
    \caption{}
    \label{fig:fp_exact_approx_mu}
  \end{subfigure}
\caption{\textit{Floating-point structure and Gaussian approximations}. (\ref{fig:fp_diag}) The structure of a floating-point number where each box represents one bit. The true bin size function $\Delta(x)$ is plotted on log-log scale for both midpoint (black solid curve) and floor quantization (blue dotted curve) with $p = 10$ and $E=4$ along with the smooth approximation $\Delta_s(x)$ (red dashed curve). (\ref{fig:fp_exact_approx_sigma}) shows the entropy of $\Xfp$ which is a discrete representation of the random variable $X \sim \gauss{0}{\sigma^2}$ that has been clipped and midpoint quantized onto a floating-point representation with precision $p=3$ and various numbers of exponent bits $E$. The x-axis shows the standard deviation $\sigma$ of the underlying continuous distribution. The horizontal red line shows the approximate entropy $\Ht^0_s(p)$. The vertical dashed lines mark $\sigma = 2^{e_{\min}}$, while the vertical dotted lines mark $\sigma = 2^{e_{\max}}$ for each $E$. Notice that exact entropy closely follows the approximate entropy until $\sigma$ approaches these boundaries for each $E$. (\ref{fig:fp_exact_approx_mu}) shows the entropy of $\Xfp$ when $p = 7$ and $E = 7$, while the mean $\mu$ of the underlying continuous random variable $X \sim \gauss{\mu}{1}$ varies from $-100$ to $100$. The approximate entropy $\Ht^\mu_s(\Xfp)$ is plotted as the red dashed curve alongside the exact entropy (solid black curve) and smoothly passes through the stepwise drops in the exact entropy as $|\mu|$ increases.}
  \label{fig:fp_exact_approx}
\end{figure}

% $\Ht^0_s$ predicts that the floating-point entropy will be constant with respect to the variance of the continuous random variable, seen by the red dashed line in Fig.~\ref{fig:fp_exact_approx_sigma}. This shows that the approximation $H(X_{fp}) \approx \tilde H_s(X_{fp})$ works well for a wide range given there are few overflows or underflows (see App.~\ref{app:exact_FPN_extrafigs}), even for 2-bit mantissa when $p=3$. Fig.~\ref{fig:fp_exponents} in App.~\ref{app:FPN_app_gauss} displays a histogram of the exponents for numbers sampled from the distribution $\mathcal{N}(0,\sigma^2)$. Additionally, from Fig.~\ref{fig:fp_exact_approx_mu} we see $H(X_{fp}) \approx \tilde H^\mu_s(X_{fp})$ works well beyond values near 0, with errors remaining within $1/2$ of a bit despite oscillatory errors due to the steps in the true bin size.

\begin{figure}[htbp]
  \centering
  \begin{subfigure}{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{code/quantized_entropy_midpoint/quantized_entropy_vs_p_midpoint.pdf}
    \caption{}
    \label{fig:fp_exact_approx_p_E}
  \end{subfigure}
  \begin{subfigure}{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{code/quantized_entropy_midpoint/joint_entropy/joint_entropy_midpoint_sigx1.0_w1.0_sigxi0.5.pdf}
    \caption{}
    \label{fig:fp_joint_exact_approx_p_E_snr_2}
  \end{subfigure}
  \begin{subfigure}{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{code/quantized_entropy_midpoint/joint_entropy/joint_entropy_midpoint_sigx1.0_w1.0_sigxi0.01.pdf}
    \caption{}
    \label{fig:fp_joint_exact_approx_p_E_snr_100}
  \end{subfigure}
\caption{\textit{Regimes where the approximations hold}. (\ref{fig:fp_exact_approx_p_E}) Shows the exact discrete entropy of $\Xfp$ as $p$ varies for each $E$ when the underlying continuous random variable is $X\sim \gauss{0}{1}$. The approximation $\Ht^0_s(p)$ is also plotted as the dashed red line. Notice that the curves for $E \geq 4$ are directly on top of each other, showing that $\Ht^0_s(p)$ is close to $H(\Xfp)$ when $E$ is large enough to keep the probability of overflows and underflows low (see App.~\ref{app:exact_FPN_extrafigs}). The approximation stays close to the true entropy with a large exponent and low precision. (\ref{fig:fp_joint_exact_approx_p_E_snr_2}) Shows the joint entropy of $(\Xfp, \Yfp)$ where $X \sim \gauss{0}{1}$, $\xi \sim \gauss{0}{0.25}$ and $Y = X + \xi$. The approximation $\Ht_s(\Xfp, \Yfp)$ is the red dashed line, and it again follows closely to $H(\Xfp, \Yfp)$ for $E \geq 4$. (\ref{fig:fp_joint_exact_approx_p_E_snr_100}) shows the same quantities as Fig.~\ref{fig:fp_joint_exact_approx_p_E_snr_2}, except $SNR \triangleq w^2\sigx^2/\sigxi^2 = 10000$ as opposed to $4$. In this high $SNR$ regime, the $\Ht_s(\Xfp, \Yfp)$ underestimates $H(\Xfp, \Yfp)$ for $p \leq 6$ due to the quantization noise that is present when the precision is low. Like the other settings, $\Ht_s(\Xfp, \Yfp)$ follows closely to $H(\Xfp, \Yfp)$ when $p >6$ and $E \geq 4$. Corollary~\ref{cor:joint_ent} reviews the exact calculation of the discrete entropy for the bivariate Gaussian case.}
  \label{fig:full_fp_exact_approx_p_E}
\end{figure}



% \subsubsection{Bivariate Gaussian} 

% We can apply a similar approach to approximating the discrete entropy for the joint entropy of $X$ and $Y = wX + \xi$ as represented over two floating-point numbers, defined by Eq.~\eqref{eq:initial_dist}. This makes use of the multivariate results presented in App.~\ref{app:FPN_app1}. For a given underlying slope $w$, by Theorem~\ref{thm:double_gaussian}, we obtain 
% \begin{equation}
%     \label{eq:approx_joint_ent_SNR}
%     \begin{aligned}
%         \Ht_s(\Xfp, \Yfp) &= 2\Ht^0_{s}(p) - \frac{1}{2} \log \bigg [1 + \frac{\sigma_x^2 w^2}{\sigma^2_\xi} \bigg ].
%     \end{aligned}
% \end{equation}

% This expression in general depends on $w$, and if $w \neq 0$, then the discrete entropy will in general be lower than $2 \Ht^0_{s}(p)$, to a degree determined by the signal-to-noise ratio $\snr = \sigma_x^2 w^2/\sigma_{\xi}^2$. One issue to notice is that for an infinite signal-to-noise ratio the expression diverges, similar to an infinite capacity scalar Gaussian channel \cite{CoverThomas, shannon_communication_1949}. This is because Eq.~\eqref{eq:diff_approx} only applies for distributions which are sufficiently broad with respect to the bin size. For infinite signal-to-noise ratio, the distribution will be a sharp line in the joint space, which will vary quickly over individual bins, making approximation 1 inaccurate. 

% This is seen in Fig.~\ref{fig:fp_joint_exact_approx_p_E_snr_100} where the dashed line showing the approximation only closely follows the exact joint entropy once the precision $p$ is $7$ for a signal-to-noise ratio of $10000$, while for a signal-to-noise ratio of $4$ Fig.~\ref{fig:fp_joint_exact_approx_p_E_snr_2} the approximation closely follows the exact joint entropy once the precision $p$ is $2$. In particular, the approximation underestimates the exact entropy in the high-$\snr$ small-$p$ regime. When there is infinite $\snr$, $X$ is perfectly recoverable from $Y$. Nonetheless, depending on the slope $w$ and the precision $p$, there could be two different $(\Xfp)_1$ and $(\Xfp)_2$ where $(\Xfp)_1 \neq (\Xfp)_2$, but $(\Yfp)_1 = Q(wX_1 + \xi_1) = Q(wX_2 + \xi_2) = (\Yfp)_2$. This would mean $(\Xfp)_1$ is not perfectly recoverable from $(\Yfp)_1$ even in the infinite-$\snr$ case. This additional entropy from the discrete binning in the  high-$\snr$ small-$p$ regime cannot be captured by the smooth approximation $\Delta_s(x)$.

% Not only do these approximations show close correspondence with the true entropy of floating-point quantized Gaussian random variables, but they can be numerically evaluated quickly for large $p$ and $E$. This contrasts the formulas for the exact entropy in Corollary~\ref{cor:gauss_fp_ent} that require the enumeration of $2^{p+E}$ values. For example, a IEEE-754 single-precision floating point number uses $p=24$ and $E=8$ which would require the enumeration of $2^{32} = 4.3\times 10^9$ values.
















